On the Limit Performance of Floating Gossip

In this paper we investigate the limit performance of Floating Gossip, a new, fully distributed Gossip Learning scheme which relies on Floating Content to implement location-based probabilistic evolution of machine learning models in an infrastructure-less manner. We consider dynamic scenarios where continuous learning is necessary, and we adopt a mean field approach to investigate the limit performance of Floating Gossip in terms of amount of data that users can incorporate into their models, as a function of the main system parameters. Different from existing approaches in which either communication or computing aspects of Gossip Learning are analyzed and optimized, our approach accounts for the compound impact of both aspects. We validate our results through detailed simulations, proving good accuracy. Our model shows that Floating Gossip can be very effective in implementing continuous training and update of machine learning models in a cooperative manner, based on opportunistic exchanges among moving users.

==> 10.draft.tex <==
\newpage
\section{Brainstorming material and extras}
\subsection{note for numeval}
Case circular and concentric ZOI and RZ. Random direction MM.
The mean length of a chord of the RZ passing through the ZOI is 
\[\frac{4}{\pi R^2}[R^3-(R^2-r^2)^\frac{3}{2}] \]
The mean length of a chord of the ZOI is $4\frac{r}{\pi}$.
The mean residual trajectory is thus 
\[
\frac{2}{\pi}(r+\frac{R^3-(R^2-r^2)^\frac{3}{2}}{R^2})
\]
Thus the mean residual time is 
\[
\bar{t}_r(R)=\frac{2}{v\pi}(r+\frac{R^3-(R^2-r^2)^\frac{3}{2}}{R^2})
\]
Where v is node speed. Similarly, the mean time spent in the ZOI is   
\[
\bar{t}_{ZOI}=\frac{4r}{v\pi}
\]

\subsection{A sample use case}

Assume that a number of users visit a large sports center, or a large shopping mall, or in general a location where many options and services are available. This location, in order to improve customer experience and satisfaction, enables users to optimize their planning choices (e.g., which attractions to visit and in what order, what to eat and where), based on official information complemented with users' opinions (both their own, or those of other users). The generation of personalized recommenNtions for user choices is based on the application of a ML model to a Ntaset residing on user devices, and in principle different for each user. The ML model is obtained upon request by users from the location manager, together with official information, while the Nta set progressively incorporates other users' opinions, which are collected with opportunistic communications through a FC scheme.

The populated ML model (i.e., the users' own model populated with opinions) is made to float via FC within a region (called replication zone or RZ) roughly coinciding with the location, in order to enable users to exchange their model versions and fuse them.  

In more detail, when in the RZ, a user downloads a stanNrd ML model, which is progressively refined by fusing the user's own model with other users' models retrieved via opportunistic exchanges. The user's own model is instrumental for the generation of decisions through local computation, and is improved by merging with different model versions obtained from other users. In addition, the user's own model is refined by acquiring more information about the system through new opinions (that we term \emph{observations}) that are collected at random times by random subsets of users. 

Thus, the user's own model evolves by merging with other models, and training due to the acquisition of new information. Both of these operations require local computation. We refer to these two computations with the names \emph{merging} and \emph{training}.

When all the necessary choices have been made, users discard their version of the model.

The main performance metric for such a system relates to the quantity of observations that are incorporated in the user's own model, and to their freshness.





 \subsection{A special case: Stationary data generation model (interesting?)}
In this setup, we assume that data points collected by each node are drawn at random from a finite set. 
This models the case in which the process which generates the data points does not vary with time. For instance, this might be the case in which data points relate to personal preferences of a population of users, if we assume the population composition not to vary over time, or more generally, when points are drawn from a distribution which does not vary over time. 

The main consequence of this assumption is that the age of an observation does not matter.

The probability for a user to possess a given model is $a$ and thus $n a$ is the mean amount of model instances it possesses, at the mean field limit. As the amount of stored information of each instance can be at most $D$, the total amount of stored information is $n a D$.

\begin{lemma} In the stationary model, the mean amount of information made available to each user is upper bounded by the FC storage capacity of the system.  
\end{lemma}
\begin{proof} To be proven. Easy to see, but many small details have to be worked out. 
\end{proof}

\subsection{Old definition of GL learning capacity}
 
\subsection{(OLD, TO BE DISMISSED) Computing Capacity of a GC}
% Modello con capacita' infinita. Model capacity e' una misura della quantita' di info che il modello e' in grado di ricostruire, con un errore epsilon. 
% Modello funziona come un "registratore" di patterns.
% A causa del fatto che l'availability del modello non e' 1, ne' l'availability delle osservazioni, la quantita' di info registrata da un modello e' limitata.
% Qual'e' il massimo di tale capacita'?


Let us assume the quality function is a step function, and which is equal to one for $G\geq G_N$.
Specifically, let us assume that that condition must be satisfied by the incorporation rate $G$ at a time from generation equal to $\tau$.
This correspond to imposing that the quality constraint from the application is satisfied within a delay of $\tau$. In a situation awareness application, this means requiring that, at any time instant, the view of the scenario built collaboratively by the GC paradigm refers to at most $\tau$ seconds in the past with respect to current time. 

Hence, if n models are floating on a same ZOI, and using the same observations, and assuming they all have the same quality function (and thus the same $G_N$) and the same $\tau$ we can express the overall incorporation rate of the systems as
\[
n \lambda P \bar{o}(\tau)
\]

This is the mean overall number of observations which the system manages to incorporate into a model through merging and training. 
Let $C_T$ and $C_M$ be the computing cost (e.g. in terms of FLOPS -Floating Point Operations Per Second) of a training and of merging tasks
respectively. To every observation included in a model it corresponds one training. In addition, if the mean rate of arrival of merging tasks for a single node is $n\frac{g}{D}a^2(1-b)^2$, the total amount of operations per second due to merging tasks in the RZ is $nga^2(1-b)^2\pi R^2 C_M$.

Hence the overall computing power of the system which is employed to elaborate and update $n$ models at the target quality and the delay $\tau$ given is
\be\label{eq:comp_throughput}
n D\pi r^2\lambda P \bar{o}(\tau)C_T+ nga^2(1-b)^2\pi R^2 C_M
\ee

Note that this can be generalized to a generic quality function, once we specify the minimum quality required.
For the target quality, one might ask what is the maximum of the quantity in \eref{eq:comp_throughput} which can be sustained by the system (which we call \textbf{computing capacity}). To this end, we need to solve the following problem:
% \begin{myproblem}[\textbf{Computing capacity of a GC}]\label{problem:opt}
% \begin{align}
% &\nonumber\\
% \vspace{-0.3in}
% & \underset{n,R,\lambda}{\text{maximize}}\;\; n D\pi r^2\lambda P \bar{o}(\tau)C_T+ nga^2(1-b)^2\pi R^2 C_M &\nonumber\\
%  &\;\;\text{subject to}: \quad \quad&\nonumber\\
%  %& \frac{\lambda}{g V S}\frac{R_P}{R_R+R_P}< 1\\
%  %& \frac{g\sum_{i=1}^{m}\sum_{j=0}^{m-i}P(i)P(j)\int_{\tau=0}^{\infty}T_{tx}(i+j,\tau)f_\tau}{G(m)}\leq D\\
%  %& \delta\pi a_R R_R R_P\leq\frac{M}{L}\\
% % & a_R=\left(1-\frac{\alpha}{g S}\frac{R_P}{(R_R+R_P)R_R}\right)\\
% % & a=1-\frac{2\alpha T_S}{DRSb}\\
% % & b=K-\sqrt{K^2-1}\\ 
% % & K=1+\frac{D}{4gT_S}+\frac{\alpha}{4gR}\\
% & n\frac{g}{D}a^2(1-b)^2 T_M \leq 1\;& \label{constraint:space}\\
%  &\text{Equation}\;(\ref{eq:ps}),\;(\ref{eq:avail_observations_22})&\nonumber\\
%  & a=1-\frac{2\alpha T_S(a)}{DRS(a)b}&\label{constraint:am}\\
%  & a > 0 & \label{constraint:fl}\\
%  & R\geq  0&\\
%  & n\geq  1&\\
%  & \lambda\geq  0&\\
%  & \bar{o}(\tau)>0& 
%  %& 0\leq L\leq M \\
% %& 0\leq \gamma\leq  \frac{DM}{L} &\label{constraint:delta}
% % & Equation \eref{eq:s_multizoi}\\
% % & 0\leq \rho\leq 1\\
% % & 0\leq S\leq 1\\
% \end{align}
% %\end{equation}
% \end{myproblem}

%Note that there is no condition for having an observation fluctuate indefinitely. This means also that, in principle, observations could get lost after some time, seen that what matter is 
% Constraint \ref{constraint:fl} requires that all of the $n$ models manage to float indefinitely over time. Constraint \ref{constraint:am} and parameters within are derived from \thref{th:steady_multi}.

\subsubsection{Approximated solution (an upper bound which should be tight)}

Let  

\[
P=\min\left(1, \frac{\bar{t}_r(R)(1-n\frac{g}{D}a^2(1-b)^2 T_M)}{T_T}\frac{1}{n\lambda \bar{t}_{ZOI}}\right)
%\min\left(1,\left \lfloor\frac{t_r(1-r T_M)}{T_T}\right \rfloor\frac{1}{q_o}\right)
\]
Thus, the objective function becomes the minimum between
\[
n D\pi r^2\lambda \bar{o}(\tau)C_T+ nga^2(1-b)^2\pi R^2 C_M
\]
and 
\[
D\pi r^2 \bar{o}(\tau)C_T\frac{\bar{t}_r(R)(1-n\frac{g}{D}a^2(1-b)^2 T_M)}{T_T\bar{t}_{ZOI}}+ nga^2\pi R^2 C_M
\]
Both functions are monotonic increasing with R. For large enough R, both functions become monotone increasing function of n too.
The max value of $n$ is the one which satisfies constraint (\ref{constraint:space}) with equality.
Thus the objective function becomes
\[
\frac{D}{T_M}(1-b)^2\pi R^2 C_M
\]
and the computing capacity per unit surface is $\frac{D}{T_M}(1-b)^2 C_M$.




% Given the system parameters, the 

% ven the system parameters, one might characterize 


%  find the minimum R and $\lambda$ such that the mean age of the model is below a given target value. 




% In this work we aim at characterizing the limit performance of the system. 

% A possibility is to evaluate how many models can be supported (as a function of their age, of their minimum quality $Q_0$, of model size L, $T_M$, $T_T$, $\lambda$, of node density and speed, of ZOI size, of the radius R of the RZ), or the max of the product of the number of models per mean model quality (for $\tau\rightarrow\infty$). This latter is the closest to the notion of capacity of the system, as it indicates the maximum amount products of the collaborative computing which the system can produce.    



% Capacity of the system can be seen as:
% \begin{itemize}
%     %\item max n of models which the system can support, when they all respect the Nyquist minimum sampling rate condition.
%     \item max $D_{min}$ which can be supported, with a single model;
%     \item maximum aggregate computing rate (training and merging)%: adding more node might increase linearly, until a bottleneck due to  
% \end{itemize}
% % , or
% % max $q_oT_T+\frac{g}{d}a^2 \bar{t}_{RZ}T_M$ 
% % max total computing load, or 
% % the maximum amount of training and merging per second that it can support.







 
 

\textbf{Note for debuggers}. 

\be\label{eq:solutiondde_2}
    \bar{o}(\tau)=\left\{
                \begin{array}{ll}
                  0 & \tau<d_I\\\\
                  \frac{1}{\left \lceil{a N}\right \rceil} &  d_i\leq \tau \leq d_I+d_M\\\\
                  \frac{e^{a\frac{b S(a)}{T_S(a)}(\tau-d_I-d_M)}}{\left \lceil{a N}\right \rceil-1+e^{a\frac{b S(a)}{T_S(a)}(\tau-d_I-d_M)}}& \tau > d_I+d_M
                 \end{array}
              \right.
\ee

\eref{eq:steady_aa} holds well when we are somehow close to saturation of the floating content capacity.
If this is not the case, $b$ takes extremely small values, possibly bringing to numerical problems.
Then we can make use the version of \eref{eq:steady_aa} which does not model the FC saturation.
It is given by (see e.g. old wowmom paper on FC capacity)
\[
a = 1- \frac{\alpha}{Rg}
\]
where g is the contact rate per unit area. Comparing this expression with \eref{eq:steady_aa}, we see that, far from FC saturation and with a low rate of observation generation, in \eref{eq:dde} we can substitute $\frac{b S(a)}{T_S(a)}$ with $\frac{2g}{D}$.

\subsection{Scheduling of computing tasks (remove}
\com{TODO:
\begin{itemize}
    \item remove assumption of slotted time from this subsection! Reshape algo in a way which does not require slotted time
    \item description of the algorithm uses lots of new notation which is not employed in the rest of the paper. Try minimizing it and making it coherent with the rest of the notation of the paper.
   \end{itemize}}
In this section we describe in detail the scheduling algorithm used at each node for serving the two types of computing tasks (merging and training). 
We assume time is divided into slots of equal duration $\Delta$. Let $t$ be the index of the $t$-th time slot, $n$ the unique label of the node we consider, and \com{$m\in 1,...,M$ the index of the $m-th$ model out of the $M$ \com{floating} in the given region}. 

We adopt the following notation:
\begin{itemize}
\item $LMI_m^n(t)$ is the local instance for the $m-th$ model at the $t-th$ slot
    \item $S^n$ and $O^n$ are respectively the queue for model instances received (waiting to be possibly merged), and for observations (waiting to be incorporated into local instances);
\item $MERGE(x, LMI_m^n)$ denotes the operation of merging of the instance x with the local instance of the $m-th$ model. The operation lasts $T_M$ seconds.
\item $TRAIN(y, LMI_m^n)$ denotes the operation of incorporating the observation y into the local instance of the $m-th$ model. The operation lasts $T_T$ seconds.
\item $REMOVE(x,Y)$ denotes the removal of the element x from the head of the queue Y.
\end{itemize}


\begin{algorithm}[h!]
		\begin{algorithmic}[1]
% 		\REQUIRE
% 			$\{n_{0},n_{1},...\}$: shuffled list of node's neighbors\\
% 			$T$: slotted simulation time\\
% 			$N$: number of nodes\\
		\FOR {$t=1,2,\ldots,T$}
			\FOR {$n=1,2,\ldots,N$}
				\IF {$n$ not busy computing}
				    \WHILE {$n$ not busy computing AND $S^n$ not empty}   
				        \STATE  {Let $s_m$ be the head of queue $S^n$} \com{Merge all instances at the same time, not one by one (??)}
			            \IF  {$s_m\nsubseteq LMI_m^n$}
			                \STATE {set $n$ busy computing until time slot $t+\floor{T_M/\Delta}$}
			                \STATE {$MERGE(s_m,LMI_m^n)$}
			                \STATE {$REMOVE(s_m,S^n)$}
			            \ENDIF
			        \ENDWHILE
			     \ENDIF
				\IF {$n$ not busy computing}
				    \WHILE {$n$ not busy computing AND $O^n$ not empty}   
				        \STATE  {Let $o$ be head of queue $O^n$} 
			            \IF {$\exists$ m s.t. $o\nin LMI_m^n$}
			                \STATE {set $n$ busy computing until time slot $\floor{T_T/\Delta}$}
			                \STATE {$TRAIN(o,LMI_m^n)$}
			            \ELSE
			                \STATE {$REMOVE(o,O^n)$} \com{Remove o after training or don't remove at all. In sims we don't remove observations}
			            \ENDIF 
			        \ENDWHILE
			     \ENDIF
			\ENDFOR
		\ENDFOR
	\end{algorithmic}
	\caption{Scheduling of computing tasks.}
	\label{alg:forwarding}
	\end{algorithm}



\subsection{Problem definition}

\com{Not sure we need this here. Maybe include in the next section, with the system description}


The goal of this work is to elaborate an analytical model which relates the main system parameters to the main performance parameters of a gossip learning scheme. Specifically:
\begin{itemize}
    \item when a single model is floating, what is the mean amount of 
\end{itemize}

\com{THIS WAS IN THE RELATED WORK -- To be moved elsewhere or deleted}

\com{The rest of this section may be redundant}


\com{now mention examples based on collaborative learning. But I would not like to tie the work only to the learning, as after all it is only a special case of fusion.}

The problem of \textbf{optimal sampling} is one of the key issues in  wireless sensor networks (WSN) design, and it has been well studied.
What differentiates it from the problem in the present paper is that in the vast majority of WSN, nodes are static and relay traffic of other nodes towards sinks. Thus several papers (see e.g. \cite{sun2013optimum} and related literature) consider the design of optimal sampling which takes into account the communication load that a given sampling strategy generates.

% Other candidates:
% Opportunistic computing \cite{mascitti2018service}, delay tolerant computing \cite{dtc2018}.

A WSN has to sample the physical parameter(s) of its
operational environment at discrete points where SNs are
located. Therefore, in general WSN can be viewed as a
distributed spatially discrete sampling problem (note that the
signal is also temporally discrete, because WSN sample the
environment at discrete time instances). \cite{mahmudimanesh2010reordering}

In WSN,
getting each sample requires not only the energy consumed by
the active sensing node, but also all the SNs along the route
from the source to the sink. As WSN nodes typically have very
limited energy, it is critical to gather sensor data by the
lowest sampling rate possible. Compressive Sampling  or Compressed Sensing (CS)
propose a sampling method which acquires the samples at a
lower rate. CS tries to acquire only the samples that are
necessary in constructing the original signal and to avoid extra
sampling when the signal is sparse or compressible.\cite{mahmudimanesh2010reordering}

Adaptive sub-Nyquist sampling techniques are not a new
topic in WSN. Backcasting \cite{willett2004backcasting} is a sampling technique for
WSNs which adapts the spatial sampling rate (and hence
energy consumption) to the current state of the operational
environment and accuracy requirements of the user. Regions with more
important data (higher spatial frequency) are densely populated
by active SNs. On the other hand, fewer SNs located in regions
with more redundancy (less spatial frequency) are activated.
Backcasting however applies only to fixed topologies and may not
well extend to random distribution of SNs. CS offers a more
general method and is less constrained to preconditions as
required by Backcasting. This makes CS quite universal and
very independent of network and environment specifications.

\textbf{In our work we do not consider CS, and rather consider simple, Nyquist criteria for sampling. 
Note though that our work can be (easily?) extended to include the effects of CS techniques.}

\section{OLD -- System Model}
\label{sec:system}

\subsection{Basic assumptions and definitions}

We consider a population of nodes cooperates in performing one or more ML-based tasks for the construction of a representation of the environment in which they move, according to one or more aspects. They collect data, train their own instance of the ML models, exchange and merge models when they come in proximity of each other. \textcolor{blue}{For simplicity we describe the system operations in the case of one model concerned with one aspect of the environment, but we will then also look at the case of many models evolving in parallel. Each node has an instance of the ML model that evolves through training with new observations and fusing with instances received from other nodes.}

Nodes are randomly distributed over the region, and they move according to a stationary mobility model such that, at any time instant, they are uniformly distributed within the region. 
Each node is equipped with a wireless transceiver, and a positioning system that allows each node to know its position in space.
We say two nodes are \textit {in contact} when they are able to directly exchange information via wireless communications.
With the random variable $\tau$ we denote the node contact time, i.e., the duration of the time interval during which two nodes are in contact, and with $f(\tau)$ we indicate its probability density function (pdf). With $C_0$ we denote the mean channel capacity between two nodes that are in contact.
%Let $g_i$, $i\in\{s,d\}$, denote the mean rate of contacts per unit area between static and dynamic nodes, and among dynamic nodes, respectively. 
\textcolor{blue}{We consider settings in which mean node density and transmission power are such that store-carry-and-forward is the main mode of communication. Indeed, when this is not the case, other, more efficient techniques than FC are applicable for information diffusion.}\footnote{This is not really an assumption used in deriving any result here, so why making it in the first place? we will rather state this in the numerical section.}


% Let $x$ denote a position in space and $\theta$ an angle, and let $\alpha(x,\theta)$ be the \textit{angular node flow}, i.e., the number of nodes moving in direction $(\theta, \theta+d\theta)$ across a perpendicular line segment of \textcolor{blue}{infinitesimal} length $ds$ centered at $x$, divided by $ds\cdot d\theta$.
% %, at the limit $ds$, $d\theta\rightarrow 0$ \vm{at the limit? these are already infinitesimal quantities.}. 
% Let $\alpha$ denote the \textit{linear flow}, given by 
% \begin{equation}
%     \alpha=\int_0^\pi \alpha(x,\theta) d\theta.
% \end{equation}
% %the integral of the angular flux over the interval $[0,\pi]$.
% % \[
% % \alpha=\int_0^\pi \alpha(x,\theta) d \theta
% % \]
% $\alpha$ is the rate at which nodes traverse a segment of unit length centered at $x$ in a same direction (e.g., from left to right of the segment). In order to simplify notation, in what follows we assume that the mobility model is isotropic, and hence, that $\alpha$ depends neither on the position in space of the unit segment, nor on the specific direction of the node flow. However, note that our approach can be easily extended to more general, non-isotropic mobility models.

Within the plane, we assume there exist a finite region (the Replication Zone or RZ) of arbitrary shape, and area A, over which nodes collect data (i.e., \emph{observations}). In addition, we assume that at the moment of entering the RZ, nodes possess a \emph{model}) which enables them to take informed decisions (for example, a map of the resources available and of the issues present in the disaster area). With $\alpha$ we denote the mean rate at which nodes enter the RZ, and we assume it to coincide with the mean rate at which nodes exit the same area.  
%\footnote{e.g. in order to perform tasks such as support disaster victims, join attractions, or take autonomous driving decisions.}. We call such tool a \textit{model}.

%We assume that each model is made available within a sub-area of the considered region of the plane (the \textit{replication zone} or RZ) which fully contains the ZOI, by means of FC.\footnote{why not through infrastructure?} 
When in the RZ, nodes exchange their instances of the model by means of opportunistic communications, following the FC paradigm. \com{Let $L$ be the model size in bits}. We assume that each node can be involved in an exchange of models with at most one node at a time. That is, whenever two nodes come in contact, they remain unavailable to further exchanges with other nodes (i.e. they are in the \textit{busy} state) until they are done exchanging models among them, or until they are not in contact any more. The order of model transfers between two nodes is assumed to be random. 

\subsection{Data generation and collection model}

%\textbf{Landmark-based.} In this model, within the ZOI there are M landmark areas (LA$_i , i=1, \cdots ,M$), fully contained within the ZOI, of arbitrary size and shape, and arbitrarily distributed. \footnote{ In autonomous vehicle driving scenarios, the tasks for which ML support is required could be, for instance, recognizing potential dangerous conditions specific for that region inside the ZOI (due for instance to the particular structure of the road), while the LA might denote the area within which data about past dangerous events and traffic patterns is made available (for instance, through broadcast from a fixed infrastructure, such as roadside units). Another example is the case of robot operation areas in a manufacturing plant. A further example is given by personalized recommendation systems. In this case, we assume that the ZOI is an area in which users make some experience (such as visiting an attraction) from which they derive an evaluation. As usual, these evaluation are very personal, and correlate with a set of factors (e.g. age, gender) but also with other preferences in other dimensions (e.g. reading habits, or music tastes). Training a model with all such these personal data, together with the evaluation, could allow other users to predict quite accurately what are the attractions he or she might appreciate the most.} %or attractions in a theme park. 
%Whenever a user enters one such landmark area $l$ at time $t$, a new observation $d_{l,t}$ is produced and stored by the user in its local memory. \footnote{Each observation may stand for a set of data representing, e.g. the robot status, or the crowd waiting to access the attraction, or the personal data of the user together with its evaluation of an attraction just visited.}
%We assume that observations are generated at a given mean rate $\lambda_m$ by a random subset of the nodes inside the RZ. 
%In this model, each user within the ZOI collects observations at a given mean rate $\lambda_m$, for the whole duration of its presence within the ZOI. 
We assume that observations are generated within the RZ according to a Poisson arrival process with rate $\lambda_m$. Every event of observation generation involves a random subset of the nodes within the RZ, which receive each a copy of that observation. 
\textcolor{blue}{how do we decide the size of such subset?? What does this model?}

%\com{Each observation is denoted with $d_{t}$, where $t$ is the time at which the observation is generated.}

\com{In this way each node, during its sojourn time on the RZ, builds its \textit{local dataset}, composed by all the observations generated in its trajectory within the RZ.} 
%Note that observations are samples of a process over time and space. In what follows, we assume that such process is not stationary. 

\section{0LD --- The gossip computing (GC) scheme}
\label{sec:GCscheme}

%\textcolor{blue}{VM: \it I would present GC before system model}
%Specifically, with each model $n$ is associated a ZOI$_n$, and an area (called \textit{replication zone} $n$ or RZ$_n$), 
%\footnote{\com{Models are delivered to users when they enter the RZ (possibly through a fixed infrastructure). G: hard to justify distributed serverless training, then. Note that we need FC only when we have multiple, non overlapping ZOIs}} 
%We assume that there exist $N, N\geq 1$ ML \textit{models} in the given region, each associated with the given ZOI. 
%Each model is fully characterized by a set of coefficients, which is function of the specific architecture and ML technique adopted. We denote with $L_n$ the total size (in bytes) of the set of coefficients for the $n$-th model ($n=1,\cdots ,N$).
%in the multi RZ scenario (only), because RZ limits the degree of overlapping among RZ and thus the amount of model replications done via opportunistic communications. order to limit We could eliminate altogether FC from the scenario, as models are delivered by the infrastructure. But then why not letting the infrastructure do all the training and update of the model, too?
%We assume each observation is uniquely identified by the LA index to which it pertains, and by the time at which it has been generated.

We consider the case in which the model is created and updated based on the data (observations) collected in the RZ. For instance, the model could be the result of a data fusion process or, as in gossip learning, be a ML model trained over the observations in the RZ.
Furthermore, as the underlying process which generates the data is non stationary, we assume that the model needs to be constantly updated according to the most recently collected data, in order to be useful. \com{these requirements should be formalized}. 

In this work, we assume such model is built collaboratively by nodes in the RZ. In order to describe the process of model building and updating, we introduce some definitions. Note that they are inspired by GL terminology, but they can be generalized to other tasks of collaborative elaboration (e.g. sensor fusion, or signal reconstruction) based on sensed data.\\
\com{
\begin{itemize}
    \item define model.
    \item define instance (existing def is not ok).
\end{itemize}}

\begin{definition}[Model instance] \textit{Given a model, an instance of the model is identified by its training set, i.e. the set of all observations which have been used to derive the coefficients of the model}. 
\end{definition}

In particular, each node maintains a \textit{local model instance}, generally different from that of other nodes. 

\begin{definition}[Training]\textit{ The model training operation is a transformation which takes as input an instance, and a set of observations, and it gives as output a new instance, with a training set given by the union of the training set of the input instance and of the set of observation.}
\end{definition}

The specific process by which the new set of model coefficients are derived depends on the model used, and it is out of the scope of this work. 
In what follows, we assume that the time taken to train a model over a set of observations is linear in the number of observations, although this assumption can be easily relaxed without significantly changing our approach. Thus, for the sake of simplicity we assume that every training task takes as input a single observation.

%\com{This definition of training assumes that it is not possible to train an instance over several data points at the same time. For the purpose of modeling the impact of training on computational load at every node, this amounts to assuming such load to be a linear function of the amount of data points to be incorporated.} \footnote{Is this realistic (e.g. in ML model training)? I guess it is a good approximation of reality.}
The \textit{age} of an observation is the time since its first incorporation into a model.
%For ease of treatment, \com{we assume all observations require the same time to be incorporated in the node's model instance}, although this assumption can be easily relaxed without significantly changing our approach.\\
Another key operation is \textit{merging}.

\begin{definition}[Merging] \textit{The merge operation is a transformation which takes as input two or more instances of a same model, and it gives as output a new instance, whose training set is the union of the training sets of all of the input instances.}\footnote{Again, the specific process by which the new set of model coefficients are derived is not specified here. Typically, they are derived through a weighted average of the coefficients of the merging model instances, though more complex approaches are possible. Such a definition of the merging operation seems to suggest that it produces a model instance with the same performance (e.g. in terms of accuracy) as a model instance obtained by training over the union of the two training sets. However this is well known to be an approximation, and \com{more accurate models could be used here (that can be the case if we use any performance metric related to the specific task which the ML must be used for)}.Non-ideality of the merge operation could be modeled with a subsampling of the set of samples included in the merging model instances. This might introduce some tradeoffs (in some case better not merging. Then when to merge?) and maybe, make still useful exchange of data instead of only models, and/or "training delegation" (i.e. sending models to neighbors to get them trained on their data). I would put this out of the scope of the paper.}
\end{definition}
Every time a node produces a new observation, he uses that new observation to train the instances of the corresponding models he possesses.
As a result, in general a fraction of the observations within a training set are endogenous, i.e. incorporated in the instance through training by the node on which they reside, while the others are exogenous, that is, incorporated through merging. In this work, we assume that that two instances with a same training set are indistinguishable, independently on whether the observations are endogenous or exogenous \footnote{In many learning problems, training and merging generally produce different models. However (e.g. see comparison between centralized and federated learning) it has been shown that these models have comparable performance in terms of accuracy. \com{We could base on this ground our choice of giving priority to merging over training, as merging costs less than training but gives same performance.}}.

Model exchanges take place whenever two nodes come in contact of each other. Merging occurs after an exchange, if the newly received model instances incorporates observations that were not present in the local model instance.
We assume that each node can perform only a single computing task at at time (training or merging), that merging tasks take precedence over training tasks, and that within each class of tasks (merging and training) the order of execution is random. 

%\com{MAM: why not? G: this is empirically shown. Otherwise, centralized ML and FL would have exactly the same performance, which is well known not to be the case. Instead, the two architectures give as output models which differ in their performance (and FL may perform better than centralized ML, in some circumstances). 

Thus, the local model instance can be trained, exchanged with other users, and merged with other model instances.
For each of the models floating in the RZ, in addition to the local instance, each node possesses a \textit{default instance}, elaborated in an offline fashion (thus without incorporating any data point, but only a-priori general knowledge). The default instance, which we assume equal for all nodes, is what each node uses when a local instance is unavailable (that is, when the node did not receive yet an instance for a given model). Being present at every node, and incorporating no observation, it is never exchanged or merged. When a node gets an observation without possessing a local instance for a model, it incorporates the observation into the default instance for that model by training, producing in this way a local instance. As a result, training occurs whenever a node obtains a new observation.

%\footnote{\com{MAM: random or irrelevant? G: I do not think it is irrelevant, in the same way as it had an impact in the traditional FC scheme. Even if better strategies can be designed however, I would leave the optimization of these out of the scope of the present work.}}.

Within the RZ, each model is trained in a collaborative fashion, over the observations collected in the RZ by nodes.
%We assume that the set of data which are relevant for its training consists in all the observations produced in the ZOI associated to that model.
%Every user entering RZ receives a basic version of each floating model, even without possessing any observation. 
Users exiting the RZ discard all models floating within it, as well as all observations. %\textbf{Why do we need this?} }  %\footnote{\com{Can a LA pertain to different ZOIs and therefore to different models? If this is the case, I am not sure a user can discard observations which have a "multiple use" when exiting a RZ. How to fix this?. Another possibility would be never discarding observations. MAM: or we could make our life simpler by describing the system in the case of just one model.}}. 
%When a user produces its first observation, for each ZOI$_n$ he is in, he elaborates a local \textit{instance} of model $n$, whose coefficients are obtained by training over that observation. Similarly, 
% Let us assume each observation to be described by a unique identifier.
% In general therefore, a local model instance is identified by the set of model coefficients,  %\footnote{\com{MAM: do you mean the initial model coefficients which a user receives when entering the RZ? otherwise, model coefficients should change at every training. G they do change at every training. here I am just defining what identifies a model instance.}}
% plus the set of identifiers of the observations on which it has been trained (henceforth denoted as \textit{training set}). 
When a user receives an instance of a model from another node, 
%if it possesses already another instance of the same model, 
it merges it with its local instance, if it has one. \com{Otherwise, it makes it its own local instance.}
%That is, it elaborates a new model instance, with a new set of coefficients (typically derived through a weighted average of the coefficients of the merging model instances, though more complex approaches are possible) and a training set consisting in the union of the training sets of the instances which have been merged. 
%MAM: I still do not understand. One model is trained on the set of observations O1, the other on O2. When the first model receives O2 \com{G: nodes exchange models, not observations!!! Observations travel and diffuse only "inside" a model instance, by affecting its coefficients.}, it will train on the observation it is missing (this is the merging operation). As a result it is trained on the union of O1 and O2. Is this not the case?}. 
We further assume that when the training set of one of the merging instances is a subset of the training set of the other merging instance, the instances are not merged, the one with the smaller training set is discarded, while the other is stored and exchanged by the node. \footnote{(this assumption is not used in the model, though maybe it is in the simulations) NP: It is used in the simulations.}
%\textbf{After a merging operation}, if the training set of the merged model does not include all the observations possessed by the node, the merged model is trained. MAM: how can we train if we do not exchange observations? We can only merge, if observations are not transferred. 
%\com{We need more clarity on what is training (this should be the incorporation in the local model of one or more observations, and if we do not exchange observations it is an operation only local to the observer) and what is merging (this is an operation that mixes two models into one, with no observation involved).}. \com{If merge costs zero, it makes sense to merge before possibly training. Otherwise it might not always be the optimal choice (the later you train, the higher the chance there will not be enough time to finish training and thus include the new observation in the model instances which are floating around, with negative impact on mean age)}. 
%as well as the order of model merging and training within each node  


\subsection{Scheduling of computing tasks}
\com{ok for keeping this section and the algorithm, as it helps clarity. Some of the considerations on the inner working of this algorithm, made in the previous part, could actually follow the presentation of the algorithm, or they could be eliminated to avoid redundancy.}
In this section we describe in detail the scheduling algorithm used at each node for serving the two types of computing tasks (merging and training). 
We assume time is divided into slots of equal duration $\Delta$. Let $t$ be the index of the $t$-th time slot, $n$ the unique label of the node we consider, and $m$ the index of the $m-th$ model floating in the given region. We adopt the following notation:
\begin{itemize}
\item $LMI_m^n(t)$ is the local instance for the $m-th$ model at the $t-th$ slot
    \item $S^n$ and $O^n$ are respectively the queue for model instances received (waiting to be possibly merged), and for observations (waiting to be incorporated into local instances);
\item $MERGE(x, LMI_m^n)$ denotes the operation of merging of the instance x with the local instance of the $m-th$ model. The operation lasts $T_M$ seconds.
\item $TRAIN(y, LMI_m^n)$ denotes the operation of incorporating the observation y into the local instance of the $m-th$ model. The operation lasts $T_T$ seconds.
\item $REMOVE(x,Y)$ denotes the removal of the element x from the head of the queue Y.
\end{itemize}

\textcolor{blue}{VM: \it Sections~\ref{sec:system} and \ref{sec:GCscheme} need to be reshaped to systematically address the definition of the scheme first, and then the system (and I would keep the model out of here). The presentation of the two components is now twisted.}


\begin{algorithm}[ht!]
		\begin{algorithmic}[1]
% 		\REQUIRE
% 			$\{n_{0},n_{1},...\}$: shuffled list of node's neighbors\\
% 			$T$: slotted simulation time\\
% 			$N$: number of nodes\\
		\FOR {$t=1,2,\ldots,T$}
			\FOR {$n=1,2,\ldots,N$}
				\IF {$n$ not busy computing}
				    \WHILE {$n$ not busy computing AND $S^n$ not empty}   
				        \STATE  {Let $s_m$ be the head of queue $S^n$} \com{Merge all instances at the same time, not one by one}
			            \IF  {$s_m\nsubseteq LMI_m^n$}
			                \STATE {set $n$ busy computing until time slot $t+\floor{T_M/\Delta}$}
			                \STATE {$MERGE(s_m,LMI_m^n)$}
			                \STATE {$REMOVE(s_m,S^n)$}
			            \ENDIF
			        \ENDWHILE
			     \ENDIF
				\IF {$n$ not busy computing}
				    \WHILE {$n$ not busy computing AND $O^n$ not empty}   
				        \STATE  {Let $o$ be head of queue $O^n$} 
			            \IF {$\exists$ m s.t. $o\nin LMI_m^n$}
			                \STATE {set $n$ busy computing until time slot $\floor{T_T/\Delta}$}
			                \STATE {$TRAIN(o,LMI_m^n)$}
			            \ELSE
			                \STATE {$REMOVE(o,O^n)$} \com{Remove o after training or don't remove at all. In sims we don't remove observations}
			            \ENDIF 
			        \ENDWHILE
			     \ENDIF
			\ENDFOR
		\ENDFOR
	\end{algorithmic}
	\caption{Scheduling of computing tasks.}
	\label{alg:forwarding}
	\end{algorithm}




\subsection{model quality (useful?)}

Let us define the \textbf{model quality}, which captures the performance of the service which relies on the results of the collaborative sensor fusion, or of the ML model trained collaboratively. In general, model quality is function of system parameters, and of $G$. Let $h(G)$ denote the function which relates the mean instantaneous relevance rate to model quality. This function depends on the specific service and hence varies a lot according to the specific context. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In what follows, we consider two possible expressions for $h(G)$, denoted respectively as $h_s$ and $h_c$. $h_s$ is a step function, equal to zero for $G\leq G_N$, and one elsewhere. This quality function models the case in which the problem is to reconstruct a spatio-temporal signal (e.g. the temperature in every point of the ZOI and across time). In this case, the sensing nodes implement a form of random (in space and time) sampling of the signal within the ZOI, and $G_N$ is the minimum Nyquist sampling rate required to reconstruct the original signal.  

%In applications, it might correspond to the minimum age of the reconstructed signal (which we assume bandlimited).

With $h_c$ we model instead a generic utility function, which we assume concave and monotone increasing as a function of G.  

Given a quality function and a minimum target quality $Q_0$, another relevant metric is the mean \textbf{age of a model} with minimum quality $Q_0$, i.e. the mean value of $\tau$ required to achieve the target minimum quality (the minimum $\tau$ such that $Q_0=h(G(\tau))$).
This is key to determine how much up to date is the model with respect to the current value which the measured parameter takes in the ZOI.


\subsection{Sampling of a (continuous) function of space and time}

Let us assume that the ZOI is associated to a function $H(x,y,t)$ which gives the temperature at a given point in time t and space within the ZOI.

Let us assume that users within the ZOI take measurements of the temperature at times which are distributed at random on the time axis. Specifically, we can assume that the arrival process of temperature measurements at each user to be Poisson with intensity $\lambda_m$. Given that users are, at any point in time, distributed uniformly at random in space within the RZ (and the ZOI in particular), from the mean user density and $\lambda_m$ we can derive the mean number of samples produced in the unit time in the unit surface within the ZOI.

The system under study can be seen as a way to sample over time and in space (uniformly at random) a given parameter (e.g. temperature) within the ZOI, given by $H(x,y,t)$.


To our purpose, $H(x,y,t)$  with $t\in(t_0,....,t)$, and $(x,y)\in ZOI$ is the input required by our model to issue recommendations. Indeed, $H(x,y,t)$ may stand for any data associated to a given spatio-temporal context, and which thus generally varies over time. For our model to be trained effectively (for instance, for the model to be able to issue recommendations on what to do n minutes in the future) it must receive in input $H(x,y,t)$  with $t\in(t_0,....,t)$, and $(x,y)\in ZOI$.

However, the FM scheme means that we do not want to use a centralized system for data collection. Instead, we use a system which brings together the data collected by a set of users in a decentralized fashion, without actually exchanging the data. Thus this data is included in a shared model which is exchanged, trained and integrated collaboratively. Instead of exchanging the data in order to collaboratively reconstruct $H(x,y,\bar{t})$, users train a model which tries to predict $H(x,y,t')$ with $t'>t$ by integrating spatio-temporal samples from various users.

The fact that each observation (a sample) may not be seeded successfully, and that it usually has an availability which is smaller than 1, implies that the data integrated into a model correspond to a (random and, we assume, uniform) downsampling of the sampled signal.  

Let us consider a node and its instance of the model, with its own training set, and let $\hat{H}(x,y,\bar{t})$ be the reconstructed function, obtained by interpolation from the data points in the training set. The training set can be seen as the output of a random sampling process (in space and in time) of $H(x,y,\bar{t})$, and of the downsampling due to the floating process. If the mean sampling rate (in space and time) resulting is "high enough", 
$H(x,y,t)$ can be reconstructed without distortion, putting the ML algorithm in the best conditions to correctly predict $H(x,y,t')$. If this is not the case, to such a error in reconstructing the signal (which we could quantify, for instance, via mean squared error, i.e. by the integral of $\abs{H(x,y,\bar{t})-\hat{H}(x,y,\bar{t})}^2$ over the ZOI) it corresponds a mean error also in the prediction. In this way, given the specific features of the signal, we can derive a function which associates a given mean sampling rate to a measure of the quality of the reconstructed  signal (which does not directly maps to the quality of the prediction, though we could take it as a proxy). Here we could choose a convex monotonically increasing convex function as a cost function.

To simplify, we can assume the signals are bandlimited, and that therefore there exist a Nyquist rate (defined in the form of rate of observations per unit surface) in space and time, beyond which the distortion of the random sampling is negligible. 

For the FM system, working at (or above) such a rate corresponds to giving to each node (after some delay, given by the speed of diffusion of content) enough information to perfectly reconstruct the input and thus allow the ML architecture to work in the best possible conditions.

A question which is close to the notion of capacity, is how many models can the system support in perfect reconstruction conditions, for a given setup?  


\subsection{Another take: $R\rightarrow\infty$, i.e. no FC for models}
\label{sec:nofcformodels}

Let us assume all nodes possess a model instance, a kind of generic purpose model built from data from other channels, and/or based on analytical models. However:
\begin{itemize}
    \item all nodes entering a ZOI have only the default model, and
    \item all nodes exiting a ZOI "discard" the training set (otherwise analysis becomes context based).
\end{itemize}

We have still \eref{eq:b_model} for $b(t,R)$, as it does not depend on the notion of availability of the model. 
The expressions of $S$ and $T_s$  is obtained by the one we had in the previous case, by letting $a_m=1$.

Let $a_d$ be the mean fraction of nodes within the ZOI which have a default model.
We can write:

\be\label{eq:avail_model_inzoi}
\dfrac{d a_d(t)}{d t}=\dfrac{2\alpha}{DR_{ZOI}}(1-a_d(t))-\dfrac{b}{T_s}a_d(t)(1-a_d(t))S 
\ee
Indeed, the first term is due to the fact that $a_d$ increases thanks to the differential between nodes with default model which enters the ZOI, and those which exit. The decrease in $a_d$ is due to nodes which meet, and in which only one has a non default model. When a node with a default model receives a node with non-default model, the latter becomes the local model instance without the need for merging, thus the second term in \eref{eq:avail_model_inzoi} has no delay. 

The structure of the differential equation \eref{eq:avail_observations} for availability remains exactly the same, by changing $a_m$ with $a_d$, and $R$ with $R_{ZOI}$:

\[
\dfrac{d a_o(t_d,R_{ZOI})}{d t}=\dfrac{b}{T_s}\left((1-a_d)a_o(t_d,R_{ZOI})+\right .
\]
\[
\left . +a_d a_o(t_d-d_M,R_{ZOI})(1-a_o(t_d-d_M,R_{ZOI}))\right)S+
\]

\be\label{eq:avail_observations}
 -\dfrac{2\alpha}{DR_{ZOI}}a_o(t_d,R_{ZOI})
\ee

Bottom line, the equations change very little.
However, it might be of value to extend model merging and training outside of the ZOI, for a zone which might coincide with the RZ, for improving the performance at the expense of involving a larger area and thus more users into the FM scheme. This would bring back to the previous scheme, where $a_m$ would be the availability of non-default models within the RZ. However, if now the reason to be of the RZ is performance within the ZOI, the equation for observation availability should be adapted to model availability within the ZOI, and a new equation for availability out of the ZOI should be elaborated.





\subsection{forplots}
\be
n D\pi r^2 \frac{P_s}{T_T} C_T+ nga_m^2(1-b)^2\pi R^2 C_M
\ee

\be
n_{max}(R)\left( D\pi r^2 \frac{1}{T_T} C_T+ g\pi R^2 C_M\right)
\ee

\be
n_{max}(R)\left( r^2 \frac{1}{R^2 T_T} C_T+ \frac{g}{D} C_M\right)
\ee

\subsection{Proof of \thref{th:steady_multi} (sketched)}
\label{sec:app_th:steady_multi}

The evolution over time $a_m(t,R)$ of is described by the following differential equation (originally derived in the FC capacity paper):
\be\label{eq:avail_model}
\dfrac{d a_m(t,R)}{d t}=\dfrac{b(t,R)}{T_s(t,R)}a_m(t,R)(1-a_m(t,R))S(t,R) -\dfrac{2\alpha}{DR}a_m(t,R)
\ee
where:
\begin{itemize}
    \item $b(t,R)$ we denote the probability that a node within the RZ is busy exchanging models at time $t$;
    \item $T_s(t,R)$ is the mean duration of an exchange of models between two nodes (i.e., mean duration of the time interval during which a node is in the busy state), given by

\be\label{eq:Ts_multicont}
T_s(t,R)= \int_{0}^{+\infty} \min{\left(\tau,\frac{c(t,R)L}{C_0}+\tau_0\right)}f(\tau)d \tau. 
\ee
$c(t,R)$ is the \textit{mean} number of models which can be exchanged during a contact between two nodes. It is a function of the availability of a model within its RZ, and of the number of RZs in which the two nodes in contact are located.
%$c$ is determined as the stationary state solution of the FC equations for the models (indeed, we are not interested in the transient for the model diffusion, which we can assume has been floating for a very long time). 
\com{We use here the single RZ formula. The general formulas are those of lemma 1 and 2 of the wowmom FC capacity paper. We also assume infinite host memory.}.
When both nodes have an instance of the model, the number of model exchanged is 2. Otherwise, there is only one model which is transferred. 
$c(t,R)$ is thus given by $ 2a_m(t,R)^2 + 2a_m(t,R)(1-a_m(t,R))=2a_m(t,R)$.
\item $S(t,R)$ is the probability of successful transfer of a \textit{single} model during a contact of duration $\tau$, and it is a function of the ratio between $\tau$ and the amount of time required to transfer all exchangeable models. 
\[
    S(t,R) = \int_{\tau_0}^{+\infty}\min{\left(1,\left \lfloor\frac{(\tau-\tau_0)}{\frac{L}{C_0}}\right \rfloor\frac{1}{c(t,R)}\right)}f(\tau)d \tau
\]
\end{itemize}
The first term in \eref{eq:avail_model} is due to the end of the exchange process among two nodes in contact. Note that this exchange takes place both when the two nodes possess an instance of the model, and when only one of them possess it. However, $a_m(t,R)$ increases only in the latter case. The second term models the decrease of nodes with models due to nodes getting out of the RZ. Both terms are normalized over the number of nodes inside the RZ. 


Now let us derive the differential equation governing the evolution over time of $b(t,R)$. The variation over time is the result of the following contributions.
\begin{itemize}
    \item The first contribution is the increase in busy nodes due to nodes coming in contact and starting to exchange models. If $g$ is the rate of such contacts, and $D$ is node density within the RZ, the contribution (normalized over the number of nodes inside the RZ) is given by $\dfrac{g}{D}2(1-b(t,R))^2$. Note the factor 2, due to the fact that every contact generates two busy nodes. Note also that for a new couple of busy nodes to form, the only requirement is that both of them are not busy. \com{This assumes that their respective instances have different training sets, such that they always have to exchange their respective models.} 
    
    Note that the number of observations which have been generated in the system since its beginning do not impact the amount of time spent exchanging models by two nodes in contact 
    %\footnote{\com{MAM: If models are a set of coefficients and a set of observations, the assumption that exchange time does not depend on the number of observations made by a node looks questionable. G: I was wrong, a model instance is a set of coefficients and  a set of observation \textbf{identifiers}. Strictly speaking, you are correct. when two nodes meet, for each model they need to understand whether they need to exchange the instance. Each of the two nodes in contact, if it has a model instance, it has to send it to the other node, unless 1) the other node has another instance of the same model whose training set is a superset of the training set of the instance which it is about to send; 2) the two training sets are identical. To check 1) nodes need to exchange the full list of observations in each training set, or at least a representation of it (a list of IDs?). However, 1) is kind of corner case, and we might choose to a) neglect this case, and have anyway an exchange of models; b) not including the exchange of these training set descriptors in our model. This would boil down to assuming such list to take much less storage space than the model coefficients. For 2), one might use a hash function, so the comparison would not imply the exchange of the full list. When observations become numerous, and time is continuous, 2) is also a corner case which could possibly be neglected. Finally, training set descriptors are important to understand whether a given observation is in the training set. However, training sets could be represented with bloom filters, whose size does not increase with the size of the set (at least within some reasonable bounds). Finally, those floating services de facto never last forever, and this makes previous assumptions more reasonable.}},
    nor the probability of having a given observation.
    It only affects the likelihood that two nodes in contact have to exchange their respective models. In what follows we put this probability to 1. This approximation is more accurate when $t>>0$ (i.e. when the system has been running for a long time) and when the number of observations is large.
    \item The second contribution is given by the decrease in busy nodes due to the end of the exchange, normalized over the number of nodes inside the RZ.
 The second contribution takes therefore the form $\dfrac{b(t,R)}{T_s(t,R)}$.
 \item  Finally, the third contribution is $\dfrac{4\alpha}{DR}b(t,R)$ and it accounts for those busy nodes which move out of the RZ while exchanging models, normalized over the number of nodes inside the RZ.
\end{itemize}

The resulting differential equation for $b(t,R)$ is thus given by:
\be \label{eq:b_model}
\dfrac{d b(t,R)}{d t}=\dfrac{g}{D}2(1-b(t,R))^2 - \dfrac{b(t,R)}{T_s(t,R)} -\dfrac{4\alpha}{DR}b(t,R)
\ee

The system of the two differential equations \eref{eq:avail_model} and \eref{eq:b_model} is a special case of the one well studied in past papers (see for instance the FC capacity wowmom paper). Note that $t$ is the time from initial seeding of the model.

Moreover, note that dynamics of model diffusion are not affected by the dynamics of model training, or merging. Indeed we assume that when two nodes start exchanging models, the schedule of a model exchange does not account for the fact that new instances of the same models might be soon available due to ongoing processes of merging or training. Instead, the processes of model exchange and of model training and merging evolve independently of each other. The former is not affected by the latter, though the reverse holds.
\subsubsection{Vincenzo's observations}
\begin{align}
\begin{cases}
\displaystyle 
\dfrac{d a_{\textcolor{blue}{m}}(t)}{d t}=\dfrac{b(t)}{T_s(t)}a_{\textcolor{blue}{m}}(t)(1-a_{\textcolor{blue}{m}}(t))S(t)+\dfrac{\lambda_m(1-a_{\textcolor{blue}{m}}(t))}{D \pi R^2} -\dfrac{2\alpha}{DR}a_{\textcolor{blue}{m}}(t),
\vspace{3mm}
\\
\dfrac{d b(t)}{d t}=\dfrac{g}{D}2(1-b(t))^2 - \dfrac{b(t)}{T_s(t)} -\dfrac{4\alpha}{DR}b(t), 
\end{cases}
\label{eq:ode}
\end{align}

\textcolor{blue}{VM: 
I also have an alternative approach: let's use $A = a_m \pi R^2 D$ and $B = b \pi R^2 D$, i.e., the absolute numbers of nodes in the RZ, with model and busy, respectively. Let's also set $\lambda_m = 0$ for the moment and assume that busy time is only for model exchange (i.e., let's neglect the busy time due to preliminary handshakes). 
The variation of $A$ is given by: $(i)$ the number of nodes that are busy and without the model, for which it takes $T_s$ to obtain a model with probability $S(t)$, and $(ii)$ the number of nodes that leave the RZ in a time unit and have the model. Since the total number of nodes in the RZ is $\pi R^2 D$ and the number of nodes that leave the RZ in a time unit is $2 \pi R \, \alpha$, we have: 
%
\begin{align}
    \dfrac{dA}{dt} & =
    \left(\pi R^2 D\right) \dfrac{b(t) \cdot \left( 1- a_m(t)\right)}{T_s(t)} S(t)- 2 \pi R \, \alpha \, a_m(t) \nonumber \\
    \Rightarrow \dfrac{da_m}{dt} & =
    \dfrac{b(t) \cdot \left( 1 - a_m(t) \right)}{T_s(t)} S(t) - \dfrac{2 \, \alpha}{R \, D} a_m(t)
\end{align}
%
\textbf{The key approximation here---as well as in the derivation of the ODEs done by Gianluca---lays in considering as independent the probabilities of being busy and having a model. Howerer, we explicitly express $a_m$ as a function of $b$ in the ODEs! Can we check this assumption with simulations?}
\indent
The variation of $B$ is due to: $(i)$ a busy node becomes idle in $T_s(t)$, $(ii)$ a busy node leaves, which makes also the paired busy node idle, and $(iii)$ two non-busy nodes meet, only one of which with a model to pass to the other node: 
%
\begin{align}
    \dfrac{dB}{dt} & = - \dfrac{B}{T_s(t)} 
    - 2 \cdot 2 \pi R \, \alpha \, b(t) \nonumber \\
    & + 2 \cdot \pi R^2 g \, (1-b(t))\, a_m(t) \cdot (1-b(t))(1-a_m(t)) \nonumber \\
    \Rightarrow 
    \dfrac{db}{dt} & = - \dfrac{b}{T_s(t)} 
    - \dfrac{4 \alpha}{R\,D} b(t) + 2 \dfrac{g}{D} \, (1-b(t))^2\, a_m(t) \, (1-a_m(t)) 
\end{align}
\textbf{Note: differently from the ODE on $b$ derived by Gianluca, my ODE makes $b(t)$ depend on $a_m(t)$, which implies that the busy probability depends on the probability of having a model. I would conclude that, e.g.,  the joint probability to be busy and have not a model is NOT necessarily $(1-a_m(t))\cdot b(t)$, which is what we use in the ODE for $a_m$. In general, all ODEs reported above and used in the past are wrong (well, let's say that they include a strong approximation).
}
%
\indent
CAUSALITY-BASED INTUITION (does it make sense to use it?): 
%
\begin{align}
    & \text{Pr}(\text{a node has (not) a model} \mid \text{the node is (not) busy}) \nonumber \\
    & \qquad = \text{Pr}(\text{a node has (not) a model}) \nonumber \\
    & \text{Pr}(\text{a node is (not) busy} \mid \text{the node has (not) a model}) \nonumber \\
    & \qquad \not = \text{Pr}(\text{a node is (not) busy}) \nonumber
\end{align}
}



% \section{System Model}
% \label{sec:system}

\subsection{Notes}
\begin{itemize}
    \item The ZOI exists in order to be able to change the parameters of FC (the RZ radius) without affecting the amount of landmark areas whose observations the model must include. However, given the use of MF model, and unless we use some geometry, performance will be based on parameters (model availability, observation availability) which are averages over the whole RZ.
    \item This can be slightly improved by having a model with two observation availabilities: One for inside the ZOI (on which we would compute performance parameters such as freshness: Indeed, the ZOI is where the model must be used), and the other for the ring around it. 
\end{itemize}

\subsection{Noelia's notes }

Within the RZ, The pieces of information to exchange between nodes are Models. These models will be always exchanged at any given opportunity at nodes encounters inside the RZ but they will only be improved (passed to the next level) if nodes have something new to contribute.

To track this information we will use a data structure belonging to the Model instance that stores each time stamp at which the model reached a new level and who performed that update in the model (e.g.,[time slot, node ID]), this data structure is shown in \ref{lst:contributions}. In this way, whenever a node receives a model instance it will check whether it has something new to contribute or not and act accordingly. We can control when a node is suitable for model training based on two different parameters: 
\begin{itemize}
    \item By working with information of new events/observations, such as node's visits to a predefined landmark. When a node passes by certain point of interest we assume it will retrieve new data that can be useful for the model, therefore this node will execute a model training.
    \item By measuring the time of the last contribution of a node to a specific model. If the last time a node contributed in a model is larger than n slots, then we can assume it has some new information to help improve the model and take it to the next level. Otherwise, the node will replace its stored model for the model received and keep it as it is (not updating it). 
\end{itemize}


The level of each model instance is measured according to two complementary indicators. Both indicators can be obtained from our previously defined data structure \ref{lst:contributions}.
\begin{itemize}
    \item On one hand, in amount of contributions to the model, also seen as trainings. When two nodes meet and both of them posses the model their lists of contributions will be merged. Nodes will discard their previous model and store the new version.
    \item Based on the freshness of the model, i.e. when two nodes possessing the same model meet they could be interested in preserving only the model that has been updated more recently.
\end{itemize}


To carry out the previous process we need to define two parameters. First, (already implemented in the simulator) the size of the model. The size of the model will directly impact the length of connections between two nodes, i.e. for how long two nodes will be busy with a transfer. On the other hand, we also need to take into account the number of slots required to do the "computation of the task" after a node receives a model (this is a new feature). It is important to note that nodes will be eligible as good peers to exchange model with whenever they are not busy. Nodes are busy only when they are already involved in a connection with other node. This assumption allows nodes to accept requests from other peers while executing a task previously received. If a node connects to a peer and exchange models while executing a task, the new received model will be queued for later processing. 

\subsection{Proactive FC computing scheme}

RZ and ZOI are circular and concentric. Nodes which enter the replication zone (RZ) have a set of $T$ different computing tasks, which they have to perform by the time they enter the Zone of Interest (ZOI), a region of the plane within the RZ. All nodes entering the RZ have the same set $T$. We assume nodes enter the RZ with a dataset for each of the computing tasks they have to perform. At each node $i$, for each task $t$ we assume there is a dataset $D_{i,t}$ required to perform the task. $\forall \{t_1,i_1\}, \{t_2,i_2\}$ we assume that $D_{i_1,t_1} \cap D_{i_2,t_2}=  \varnothing$ (this can be relaxed later, but it sounds like conservative).
To each of the $T$ tasks it is associated a \textit{model} $M_t$ i.e. a piece of software and data (e.g. a ML architecture with its parameters) which, together with the user data, are required to execute the $t$-th task on that user.
%Each client node entering the AZ has $T$ computing tasks, to perform by the time it enters the ZOI.
\com{How models are produced and trained is out of the scope of this work. We assume they are in a final state, i.e. they do not need further training (also because here we have no notion of model performance, if one excludes the time it takes to run.)}\\

We assume the computing tasks to be performed are related to a specific spatial context. A typical example is a computing task related to the training or the use of a ML model. In these cases, the model has been built taking into account local data and context, and it is therefore highly specific for that context itself. As we assume no static infrastructure (e.g. edge servers) can support nodes in the computation, these models only reside on nodes (both client and server) and they are made available in a region around the ZOI called the replication zone (RZ) via the FC paradigm. We denote with $L$ the size of a model, i.e. the total amount of info which has to be transferred between two nodes in order to transfer the model.

\vm{This is the first problem tackled in the approach proposed by Gianluca: make the model float, which is not much different from content floating as we have studied and published so far.}\com{Indeed, research problems are not here. This is just a component.} Nodes entering the RZ possess no model. At the beginning of the floating scheme, for each model $t$ we assume there is a subset of the nodes in the RZ which possess it. Every time two nodes meet, each model is replicated from the node who possesses it to the one who doesn't, in a random order. Nodes which exit the RZ discard the models. Nodes have infinite memory size.

As soon as a client node receives the model for the $t-$th task, it starts performing the computing task if no other task is being performed. Otherwise, it waits for the end of the task under execution to start a new one. We assume a node can perform only one computing task at a time. Let $d$ the time required to complete a task.     

The performance metric of this scheme (the \textit{success probability})is the probability for a task to be complete by the time a user enters the ZOI. If a user did not complete the task by the time it enters the ZOI, he will be forced to use cloud services and cellular communications to get it completed. 

\vm{From this point on, this seems another paper, with another research problem. Here the problem is opportunistic offloading, for which there are a lot of results in the literature. What's new here?}
\com{The novelty (small or not) is proactive computing supported by FC-enabled offloading. Offloading is only a component. The old FC scheme, in support of computing, is another (well studied) component. But the whole scheme is new (to the best of my current knowledge).}
We assume that in addition to perform computing tasks locally, using the computing resources of the node itself, nodes can offload the computing task to other client nodes, in order to maximize the success probability. This might happen when  the offloading node has significantly less tasks to complete than the offloaded (e.g. because it has already entered the ZOI), or when the offloading performs computations faster. 
Once the offloading node completes the task, we assume that the result is received instantaneously by the offloaded node, if the two nodes are still in contact. Otherwise, if the two nodes stop being in contact during model/data transfer and offloaded task execution, the offloader discards the computing task.
For this reason (i.e given the limited duration of contacts among nodes), the offloaded tasks take precedence over other tasks of the offloading node.  \vm{I'm confused. Which one is  the offloading node and which the offloader?}
\com{Offloaded node is the node whose load is taken off. The node who helps is the offloading node.}
\vm{Assuming that the offloading node is the one which takes the task and lends compute power to someone else, it is questionable that it would give priority to offloaded tasks over its own tasks. }\com{Very questionable, agree. Already this shows that it is not clear which scheduling strategy works best-an open issue. I assumed that tasks done on behalf of other nodes needs to take precedence, as contacts do not last forever, and if nodes get disconnected while the offloaded task is still not complete I assumed (but we can change this, as well as many other aspects) that the offloaded task get discarded. I am not sure this is actually optimal, in view of the main performance parameter - the mean success probability (or mean probability for a task to be executed before entering the ZOI).}

%If the offloading possesses the model for the task being offloaded, it only needs to receive the dataset from the offloading node relative to that task. Otherwise, the offloading node has to send to the offloader also the model required for that task \com{we can change this, if needed}.
%\com{(When nodes have finite memory for models, we can assume that they are allowed to discard the model for a given task when that task is completed. But let us neglect this in a first step).}
%The second class of nodes is given by the \textit{server nodes}. They do not need to perform computations by their own, but they may perform computation on behalf of client nodes, i.e. play the role of offloaders. Let $k$ be the ratio between the task completion time at client nodes and at server nodes.

At any point in time, every node can communicate with at most another node, and it cannot change the node with which it is communicating until the exchange between the two nodes is complete (i.e. the two nodes have nothing to exchange anymore, and all offloaded tasks have been completed).

The specific task and communications scheduling algorithm is as follows.
Let i and j be the two nodes in contact. 
When node $i$ is done transmitting all the models which are missing by node $j$, node $j$ updates its schedule of tasks to be executed, and computes the time at which all the tasks of the queue will be completed. As we assume to know the mean time to ZOI traversal for each node $j$, conditioned to having spent $\delta$ seconds in the RZ, node $j$ can forecast the average success probability for its own tasks. 
\vm{The forecast introduces a third problem to solve, which is orthogonal to the one of floating the model and the one of offloading the computation.}
\com{Indeed, taken seriously. But we can simplify on this dimension, by assuming (as I have assumed here, see system model) that we know the pdf of the mean time between RZ ingress and ZOI ingress. Then the "forecast" is implemented by estimating the mean time to ZOI ingress, and the time taken to complete all tasks in the queue (which we assume deterministic). }
Node $i$ performs the same forecast. 
Both nodes compute also how such forecasts would change if the node with lower forecasted success rate offloads one or more tasks to the other node, and determine the optimal number of offloaded tasks, 
taking into account the time it takes to transfer the model, and the fact that offloaded tasks take priority over local tasks. \vm{My impression is that this work would deviate a lot form what Noelia has done so far, and there will be no time to complete it before Noelia's contract ends}

\mam{My elaboration on your ideas:
Consider an area where many things happen (e.g., a theme park, like Disneyland or Seaworld, but also a factory floor or a battlefield). Over this area many actors (humans or machines) collect viewpoints of what is happening, but they only have partial information, while global information could be very valuable to make decisions (which attraction to visit, where to provide additional workforce or more soldiers). Global information can only be obtained by collecting and fusing user viewpoints that are progressively updated in the end user terminals. When terminals meet, they exchange their viewpoints and generate a fusion, which becomes more valuable because it incorporates many viewpoints, some older, some more recent. The utility of the newly generated viewpoint is a function of the number of collected individual viewpoints and of their ages. We could investigate the evolution of the average utility of viewpoints (might be called value of information). In the code of Noelia this should not be very difficult to implement. It needs only to keep track of what viewpoints are collected and their ages, so that utility can be computed at any time for all users.}




\com{\textbf{GR My elaborations over MAM.} }
With a system, where info is distributed but where no new info is produced over time, we will see the fusion gradually converging to a global view (complete or not, based on how well the single elements and the fusion float).

If we assume a (stationary) arrival process of new info which has to be fused with new one, the fusion keeps on evolving constantly.

3) if the age of info is in  (i.e, if we have a notion of users regularly producing "updates", we should have a look at  "the age of gossip" paper by JYLB. That would mark a deviation from the traditional FC scheme, as for every content may be floating in its AZ in several different versions, and a node getting two versions would keep and replicate only the most recent one.

The age of gossip paper does not consider 1) conditions for info not to disappear, as a function of system geometry (the anchor zone) and node mobility; 2)  a notion of maximum load of information which the system can support (similar to FC capacity idea ), and the relationship (trade-off) between such a maximum load and the mean age of floating information. This is to me another potential direction of work, which would elaborate on top of JYLB paper.

\subsection{Overview}
We aim at characterizing the computational capacity of a localized system where tasks are distributed to nodes and retrieved after completion in a delay tolerant manner relying only on opportunistic exchanges  among  nodes  and their local resources within  a  restricted  geographic area. The  measurement of the performance of computational tasks will be carried out according to: 

\begin{itemize}
        \item User resources: computational resources, memory, energy, etc.
        \item Opportunistic exchanges varying nodes density and mobility in the RZ.
\end{itemize}

The system will require the following prerequisites for a task execution:
\begin{itemize}
    \item 2 contacts needed: First to get the task from a peer node, second to deliver the complete task to another node.
    \vm{This is needed only if the one who passes a task wants to get a result back. But I think this is a big changes with respect to what Noelia has done so far, and it might be seen as a change of paradigm: before we wanted something to float for whoever will pass by, now we want to give everybody the possibility to offload some task of personal interest, with no benefit for the community. In addition, I think it makes analysis and simulation of the system more complex than needed if we just want to evaluate the computational capacity of the infrastructureless system.}
     \item Exchange of tasks to neighbouring nodes only, within a radius of transmission.
    \item Complete the task before leaving the RZ.
    \item Must the content/task evolve? How? It will require a number of slots to be completed and some node resources. Nodes will not have unlimited computational or memory resources so to restrict the amount of tasks that a node can perform during its visit to the RZ. \vm{Let's consider a distributed learning system. The model will evolve. However, all we need to characterize is the speed at which it evolves while floating, i.e., how many users per second get the model, manage to train it one step more, and pass it to someone else.}
\end{itemize}



More generally, what could be made to float is any combination of software applications and data which enable the execution of some computing task over a dataset belonging to each user. To our purpose, the \textit{size of the model} would be in this case the total size (in bytes) of the software components and data which need to be transferred between a node which is able to perform the computing task on behalf of the user, and a node which is not, for the latter to be able to perform the given computing task. \com{It is up to us to decide if a node which receives a model needs some time before being able to use it, e.g. to model time required for installing, configuration changes, etc.}  

\vm{This is a nice application but it seems a bit unrealistic to train a model from scratch within a few minutes (or less). There should be a model that floats in the RZ and devices passing by might look for a model to plug some parameters (e.g., their personal profile) and obtain some suggestions about what to do in the sport center. However, this would be plain floating content, with no need of computation offloading. If instead we want a user that injects a job in the system, in the form of a query, and waits for the query to float, being grabbed by someone, elaborated and answered before he/she gets to the sport center, than this makes sense but it requires the 2 contacts mentioned in the introduction. I would instead propose a slightly difffernt scenario: the potential customer retrieves a model that floats and $(i)$ uses it to get suggestions (local private computation) while at the same time $(ii)$ he/she improves the training of the model by merging different versions he/she founds and by adding extra training, for the benefit of who will arrive later. Here, if the model float, the probability to get a well-trained model before entering the ZOI is high, but even if the model does not float, each customer can re-start training and merging models, so that the metric to be used is the probability to get a well-enough trained model before entering the ZOI, even if the model eventually does not float.}

==> 9.algorithm.tex <==
\section{The algorithm}
\label{sec:system}

\com{Describe system model.}
\com{Describe data generation model.}
\com{Describe model for arrival process of computing task.}
\com{Define data structure}% Describe algorithm in (detailed) pseudo code.} 



To measure the computational capacity of the system, we can look at the number of contributions of every model replica. If we assume we work only with one model by now, at the end of a simulation run we will have several copies of the same model that evolved thought different branches and therefore will show different information in their contributions data structures. We can see, at each branch, how many times it evolved and which nodes contributed. Besides, if we assume a fix number of slots for tasks execution we also know for how long nodes used their resources for the cause, being a good indicator of the computational power used in the system.


\begin{lstlisting}[caption={Data structure representing a dictionary with the nodes contributions in a Model},captionpos=b,label={lst:contributions}]
struct {
    float timestamp;
    int node.id;
} Dict();
\end{lstlisting}

\begin{algorithm}[ht!]
		\begin{algorithmic}[1]
		\REQUIRE
			$\{n_{0},n_{1},...\}$: shuffled list of node's neighbors\\
			$S$: slotted simulation time\\
			$N$: number of nodes\\
		\FOR {$t=1,2,\ldots,S$}
			\FOR {$node=1,2,\ldots,N$}
				\IF {$node$ not busy}
				    \STATE $node.busy \gets True$
				    \COMMENT{Node become busy}
					\STATE $peer \gets n_{0}$ 				\COMMENT{Set node's peer}
					\IF {$peer$ not busy}
					    \STATE $peer.busy \gets True $				\COMMENT{Peer become busy}
						\STATE $modelExchange(node,peer)$  \COMMENT{Local $node$ exchanges Model with $peer$}
						\STATE $peer.busy \gets False$
						\COMMENT{Peer realease}
						\STATE $node.busy \gets False$
						\COMMENT{Node release}
					    \STATE $model \gets merge(localModels,recModel)$
					    \COMMENT{Merge models if node already had a local version of the received model}
    					\IF {newObservation in node}
    					    \STATE $trainModel(model,localData)$
    					    \COMMENT{Train the model with local data}
    					\ENDIF
    					\STATE $storeModel(model)$
    					\COMMENT{Store the model w/ or w/o training}
					\ENDIF
				\ENDIF
			\ENDFOR
		\ENDFOR
	\end{algorithmic}
	\caption{Model offloading and training}
	\label{alg:forwarding}
	\end{algorithm}
	
	\begin{algorithm}[b]
		\begin{algorithmic}[1]
		\REQUIRE
		    ${m_{0},m_{1},...}$: List of local models\\
			$M$: Model received\\
            \FOR {$m$ in ${m_{0},m_{1},...}$}
        		\IF {$M.id$ == $m.id$}
        			\IF {$M.contributions$ != $m.contributions$}
        				\FOR {k,v in $M.contributions.items()$}
        				    \IF{k,v not in $m.contributions.items()$}
        				        \STATE $m.contributions.add(k,v)$
        				        \Comment{Add the missing contribution to the local model}
        				    \ENDIF
        				\ENDFOR
        			\ENDIF
        		\ENDIF
        	\ENDFOR
	\end{algorithmic}
	\caption{Model merging}
	\label{alg:merging}
	\end{algorithm}

==> Noelias_numeval.tex <==
\section{NOELIA'S Performance evaluation (here in case you want to fish content, comments, details, for our work)}
\label{sec:pevaluation}

In this section, we evaluate numerically the performance of the \ac{FG} system by means of simulations. To this aim, I have used the \ac{FG} version of the \ac{FC} simulator used in the rest of the thesis, which allows to evaluate the fundamental factors that affect the learning capacity of \ac{FG}. The description of the simulator used for \ac{FG} is contained in the Appendix.

\subsection{System simulation and setup}

The simulator implements \ac{FC} for the exchange of model instances, which is done like for contents in a normal \ac{FC} systems.
For this work, we have applied a restrictive data transfer policy in which nodes can only store and exchange models while they are inside the \ac{RZ}. When nodes leave the \ac{RZ}, all models and pending models, that are queued to be trained or merged, will be erased from node databases.

In the simulations, we consider a rectangular region which embeds a single \ac{RZ}. When a new observation is generated, only one node in the \ac{RZ}, chosen uniformly at random every time, receives it. We define this node as the ``seeder'' and such node will also obtain a model instance related to such observation in case it does not posses it before observation generation time. Within the \ac{RZ}, nodes that come into contact, and are not already enrolled in another connection, will be able to connect and exchange the missing model instances in the peer node. After model exchange or observation generation, each node holds a FIFO queue of tasks (pending model instances) to be sequentially computed according to predefined merging and training times. Tasks are never dropped unless the node leaves the \ac{RZ}, but can suffer large delays before being completed.

At the beginning of each simulation run, nodes are distributed uniformly at random, then they move according to the \ac{RDMM} model, with wrap-around at the boundary of the simulation area. When two nodes are within transmission range, the channel data rate is constant over time.  
Simulated time has been divided into equally sized slots, whose duration has been chosen so as to minimize errors in detecting when two nodes are in range or when a node is within a given \ac{RZ}, according to the input parameters used in the simulations settings. 

The simulator introduces the following approximations on the behavior of \ac{FG}: for simplicity, the results reported in what follows have been computed by considering that the length of model instances do not depend on the number of observations used to train the model. Models have a predefined size and trained observations are only considered when exchanging models, i.e., a node will exchange a given model instance to a peer node only if the model instance has observations in its training set that are missing in the peer node model instance. Training time and merging time are also considered as constant values, which means that the complexity of training and merging operations is barely or not affected by the description of an observation and the structure of the model. This occurs, for instance, for distributed \ac{ML} algorithms that need to exchange and update a fixed number of parameters. Most of the times a training process will be preceded by a merging process since the most common case is that a node already possesses an instance of the same model which will have to be merged with the new received instance. It is important to note that, there is only one case in which this merging process is definitely not needed, when a seeder generates an observation and it does not possess the model instance belonging to that observation. In this specific case, the seeder will directly train a default model instance with the generated observation.

Unless otherwise specified, the simulation area is a square of side $\SI{200}{\meter}$, the \ac{RZ} has a default radius of $\SI{100}{\meter}$ and it is located at the center of the area. Observations are generated at a rate $\lambda = \SI{0.1}{obs/s}$ per model, and inter-arrival time of observations is exponential.
Each observation has a lifetime of $300$~s. Therefore, $30$~fresher observations are generated, on average, per model, during the lifetime of an observation.
The channel rate is equal to $\SI{10}{\mega\bit}/s$ when nodes are within $\SI{5}{\meter}$, and it is $\SI{0}{\mega\bit}/s$ otherwise. There are $200$ nodes in total, which makes $N \simeq 157$ nodes in the \ac{RZ} in total, on average. The speed of nodes is $0.5$ m/s. On average, the sojourn of a node in the \ac{RZ} lasts $\sqrt{2}$ times the radius of the \ac{RZ} divided by the speed, which means about $T_{\text{RZ}} \simeq 282$~s in the adopted settings. 

For model size we have chosen different values depending on three configurations, using $1$ to $10$ models, which span very different communication and computing loads. We also report results of experiments with small and large training and merging time, so as to be able to focus on communication limits (when the processing time is short) or on computing limits (when processing time is long). All the input parameters of the simulator are shown in \cref{table:computational-parameters}. 

We count on $20$ simulation runs per configuration and each run has been executed for a duration of \num{10000} time slots, which proved to be sufficient to observe the system out of any transient, and data affected by transient effects have been discarded. 

\begin{table}[t!]\caption{Input parameters}
\small
\begin{tabular}{p{0.5\columnwidth} | p{0.5\columnwidth}}
Parameter &  Value \\
\hline
Number of models ($M$)		& 1, 3, 10\\
Model size ($L$)             & \SI{0.01}{Mb} - \SI{100}{Mb} \\
Observation generation rate ($g$)  &  \SI{0.1}{obs/s}\\
Total number of users   & $200$ \\
User Speed              & \SI{0.5}{m/s}   \\
Slot length             & \SI{0.5}{s}   \\
Number of \ac{RZ}s      & 1\\
Transmission range      & \SI{5}{\meter}\\
Radius of replication   & \SI{100}{\meter}\\
Simulated area          & \SI{200}{m} $\times$ \SI{200}{m} \\  
Channel rate            & \SI{10}{Mb/s}\\
Memory limit            & infinite\\
Merging time ($T_M$)    & \SI{2.5}{s}, \SI{25}{s} \\
Training time ($T_T$)   & \SI{5}{s}, \SI{50}{s} \\
Simulation length       & \SI{10000}{slots} \\
\end{tabular}
\normalsize
\label{table:computational-parameters}
\end{table}

\subsection{Numerical results}

\begin{figure}[!ht]
\centering
\includegraphics[width=\columnwidth]{fig/model-availability.pdf}
\caption{Model availability with low training and merging times.} 
\label{f:model-availability}
\end{figure}

\cref{f:model-availability} shows the time average of the model availability $A^{(\text{m})}(t)$, computed over the last $30\%$ of the simulations, for increasing values of model size, with short training and merging times. 
In this case, for the three different configurations (with 1, 3 and 10 injected models) the model availability starts at high values, between $0.75$ and $0.8$, depending on the number of models. 
This happens because, for small model sizes, transfer times are much shorter than contact times, on average. With a model size of $10\,000$ bits, and a data rate of $10$~Mb/s, the transfer time is between $1$~ms and $2$~ms, depending on whether transmission is unidirectional or bidirectional. 

This has to be compared with an average contact time $t_c$ of about $6$~s, and an average inter-contact time ($g^{-1}$) of about $40$~s, as observed experimentally in the simulations.\footnote{Indeed, a standard analysis of the \ac{RDMM} mobility model would tell that there should be, on average $1.96$ contacts per second in the \ac{RZ}, each contact involving $2$ nodes. Thus, it will take $N/(1.96 \cdot 2) \simeq 40$~s for all $N\simeq 157$ nodes in the \ac{RZ} to be involved in a contact.}
Under these circumstances, observations are mostly acquired via model exchanges and merging rather than via direct training. Indeed, note that, with the observation generation rate of $0.1$~obs/s per model, an average sojourn time of $282$~s in the \ac{RZ}, and $157$ nodes in the \ac{RZ}, on average, each  node will receive $0.18$~obs/model while in the \ac{RZ}. Being the generation of observations a Poisson process, we also know that the probability that a node receives no observation is about $0.84$ and the probability to receive exactly $1$ observation is about $0.15$.  

With an extreme simplification, we can estimate the average model availability in the case of one model by looking at the probability of acquiring the model within the first $3$ contacts (i.e., the probability to acquire the model only after more than $3$ contacts becomes negligible).
Assuming that the contacts occur at deterministic spacing, i.e., every $g^{-1}=40$~s in our case, and accounting for time averaging, the model availability obeys the following equation:

\begin{align}
    \overline{A^{(m)}}
    &=
    \sum_{k=1}^3
    \overline{A^{(m)}}
    \,
    \left(1-\overline{A^{(m)}}\right)^{k-1}
    \,
    \dfrac{T_{\text{RZ}}-k/g-(T_M+(T_M+T_T)/2)}{T_{\text{RZ}}},
    \label{eq:approx_2nd}
\end{align}


where the merging time $T_M$ is $2.5$~s and the training time $T_T$ is $5$~s. Discounting half of $T_M+T_T$ from the available time is done to account for the fact that a merging task can be queued if the node is busy with computation when a model exchange occurs. 
After factorizing out the term $\overline{A^{(m)}}$, the above expression reduces to a second order equation with only one solution in the range $(0,1)$. In particular, for the case of the experiments reported in \cref{f:model-availability}, the solution of~\cref{eq:approx_2nd} is $\overline{A^{(m)}} \simeq 0.79$.
This result matches well enough the experimental value reported in the figure for one model. 
With more models, the model transfer and merging times grow linearly, which implies a delay in merging models, hence a reduction of time over which the models are available. This effect is indeed observed in the figure. 

At the other extreme, with very large models, contact times are not sufficiently long for model transfer. Models can only be acquired with the training of endogenous observations. 
As mentioned above, each node will receive $0.18$ observations per \ac{RZ} traversal, and each observation, in practice, will be trained into a different model since the probability to receive more than one observation per node is negligible. Considering that the observation will be received, on average, for half of the sojourn through the \ac{RZ}, and training time is negligible with respect to the sojourn time, we should expect an average model availability of about $0.09$. 
This value is very close to what we see in  \cref{f:model-availability}. Moreover, with such a short training time, the result applies independently of the number of models.

Finally, the transition between the two regimes can be expected to happen before model sizes are such that transfer times are comparable to contact times. In the case of \cref{f:model-availability}, during a contact time is possible to transfer between $30$ and $60$ Mb,  and indeed we can see in the figure that transitions happen between $6$ and $60$~Mb, in the case of one model. With more models, the transition moves to the left because of the increased volume of data to be transferred, which roughly scales with the number of models. 

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{fig/computational-capacity.pdf}
\caption{Learning capacity with low training and merging times.} 
\label{f:computational-capacity}
\end{figure}

The learning capacity that corresponds to the average model availability discussed so far is depicted in \cref{f:computational-capacity}. In the figure, the time-average of the number of observations per node is taken over the entire simulation.  The trend shown in the figure is similar to the one of average model
availability, and in particular the transition between high and low capacity regions occur like for availability metrics.
It is therefore full clear that relying on communication though an \ac{FC} system is doable under low/medium loads, and that \ac{FC} introduces a sharp phase transition on \ac{ML} and \ac{FG} performance. The impact of computing load, which in the figures discussed so far is visible in the differences between curves computed with a different number of models, is much less disruptive. 
Indeed, notwithstanding the fact that here the values reported are cumulative values over the number of models $M$, it is interesting to observe that the performance metrics do not scale with $M$ but slightly change their behavior.    
The values of $\overline{T}$ on the right part of \cref{f:computational-capacity} correspond to the equivalent values of model availability (see  \cref{f:model-availability}) multiplied by the number of models. This is due to the fact that models are only acquired by endogenous observation and training, and, as commented before, each model contains only one observation with high probability. 

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{fig/obs-availability-overtime-smallL.pdf}
\caption{Observation availability over time with short training and merging times and $L=0.01$ Mb.} 
\label{f:smallL}
\end{figure}

Instead, for low model sizes (left part of the figure), we know the average fraction of nodes with model, and we need to estimate the average number of observations per model at a generic node, so as to estimate the values reported in the figure. 

Neglecting the queuing delay of processing tasks, which is possible only for small values of $T_T$ and $T_M$ and for a limited number of floating models, 
the number of nodes at which each observation is available can be approximated as an exponentially growing function of the observation lifetime. 
More specifically, from the moment an observation is integrated in a model for the first time, which happens, on average when the node training the observation is halfway through the \ac{RZ}, the number of nodes with that observation tends to double every inter-contact time $g^{-1} \simeq 40$~s. 

However, we must account for the fact that the observation diffusion time starts with a delay equal to the merging plus training times $T_M+T_T$; besides, nodes exit the \ac{RZ} with a rate of  $T_{\text{RZ}}^{-1} \simeq 1/282$~s$^{-1}$, and hence drop all their observations. Therefore, in $g^{-1}$~s, the fraction of nodes that leave the \ac{RZ} is $1/(g\,T_{\text{RZ}}) \simeq 0.14$. This fraction applies to all nodes, and in particular to nodes with the considered  observation. Thus,  we can approximate the number of nodes with the observation, $\theta$ seconds after its generation as $0$ if $\theta< T_M+T_T$, and $\left(2 \cdot \left(1 - \frac{1}{g\,T_{\text{RZ}}}\right)\right)^{g\,(\theta-(T_M+T_T))}$ otherwise: 
%
$$n(\theta) \simeq \left(2\cdot\left(1-\dfrac{1}{g\,T_{\text{RZ}}}\right)\right)^{g\,\left(\theta-(T_M+T_T)\right)} u\left(t-(T_M+T_T)\right), \quad \theta \le \tau_l,$$ 
%
where $u(\cdot)$ is the unit step function and the expression is valid $\theta$ time units after observation generation and up to $\tau_l$.
The described behavior is reflected in \cref{f:smallL}, which reports observation availability curves as they evolve in the lifespan of an observation when the model size is small. The curves roughly correspond to $n(\theta)/(N\,\overline{A^{(m)}})$, which is an approximation for the observation availability, given the average model availability. The figure shows that, as expected, the number of models does not make an important difference in the curves, at least up to $M=10$. Indeed, consider that the average processing time required at each node can be, in the worst case the one required to merge $M\,g\,T_{\text{RZ}}$ times per \ac{RZ} traversal, plus $M\, \lambda\, T_{\text{RZ}} / N$ observation training occurrences. With the values used in the described experiments, this sums up to about $18.5\,M$ seconds, which is sufficiently lower than the total time in the \ac{RZ}, so that we can, as a first approximation, neglect the queueing delay of processing tasks.

However, for what concerns the average number of observations present in each node, we have to consider that each observation $i$ is received first by a non-seeder node when it is $\theta_i$ time units old, and then it is kept until the node leaves the \ac{RZ}. Some observations will expire during the node's journey through the \ac{RZ}, but they will be replaced by other observations received directly or by means of model instance exchanges. Thus, putting together what seen in the \ac{RZ} for an observation and its replacement after expiration, the average node sees two parts of the average observation diffusion curve for each of the $\lambda\,\tau_l$ observations per model that can be present at the same time (i.e., only observations which have not expired, hence they are at most $\tau_l$ time units old). In total, for each observation diffusion curve, the node sees an interval of time $T_{\text{RZ}} < \tau_l$. This means that, in the computation of the average number of observations contained in a model, the time-average over the lifetime of a generic observation is limited to $T_{\text{RZ}}$ rather than $\tau_l$. The missing interval is a randomly located time window of average size $\tau_l- T_{\text{RZ}}$, expressing the random \textit{gap window} in between one observation and its replacement, and over which the observation diffusion curve contributes as zero.\footnote{There could be multiple gaps, expressing the fact that an observation is replaced and then the replacement expires as well and is replaced in turn. However, the probability that this event occurs is negligible because the lifetime of an observation is typically longer than the average sojourn time of a node in the \ac{RZ}.} 
%
Under such approximations, taking per-node and per-model averages, and further averaging over the position of a gap window of size equal to its mean, we can write the following approximated expression: 
%
\begin{align}
    \overline{T}
    & \simeq
    \overline{A^{(m)}} \,M\,
    \dfrac{\lambda \, \tau_l}{N}
    \cdot 
    \dfrac{1}{T_{\text{RZ}}}
    \int_0^{T_{\text{RZ}}}
    \dfrac{1}{T_{\text{RZ}}}
    \left(
    \int_0^{x} n(\theta) d\theta
    +
    \int_{x+\tau_l- T_{\text{RZ}}}^{\tau_l} 
    n(\theta) d\theta
    \right)
    dx.
    \label{eq:T_left}
\end{align}
%
Note that the above expression sums, for each of the $\overline{A^{(m)}}\, M$ models owned by a node, the time-average of the number of observations per model received during its sojourn in the \ac{RZ} crossing time.
A numerical evaluation of \cref{eq:T_left} with $M=\{1,3,10\}$ and the corresponding model availability values of  \cref{f:model-availability} yields the following values: $2.3$, $6.7$, and $21.7$, which are decent estimates of the leftmost values of the curves depicted in \cref{f:computational-capacity}.

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{fig/obs-availability-overtime-largeL.pdf}
\caption{Observation availability over time with short training and merging times and $L=100$ Mb.} 
\label{f:largeL}
\end{figure}

As mentioned before, the diffusion of observation becomes impossible for large values of $L$. In that case, the curve of observation availability vs observation lifetime can be approximated with a step function, which is similar to the experimental results shown in \cref{f:largeL}. This behavior depends on the fact that each observation is available, after training, only at the seeder, and the number of nodes with model in the \ac{RZ} shows only small fluctuations. For the case of  \cref{f:largeL}, the average model availability is about $0.1$ (see \cref{f:model-availability}), which means about $15.7$ nodes have the model, and the observation availability, once the observation has been trained, is $1/15.7 = 0.064$, which is close to what shown in \cref{f:largeL}.  


\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{fig/model-availability-10x.pdf}
\caption{Model availability with high training and merging times.} 
\label{f:model-availability-10x}
\end{figure}


To further evaluate the impact of the computing load, the following figures report the case in which training and merging times become large and non-negligible with respect to the time spent by a node in the \ac{RZ}. To do so, the figures report results obtained in the same operational conditions as in the figures commented before, but for ten times longer training an merging times. In particular, with $T_M+T_T=75$~s, the rate of $0.18$ observations to train per second brings a load of about $5\%$ per model, which means that just training, e.g., with $10$ models, would keep the node busy for half of its journey in the \ac{RZ}. Merging tasks, at a rate of $1$ merging per model every $g^{-1}=40$~s and $T_M=25$~s would keep a node busy all the time with as few as $4$ models as soon as their availability reaches $0.4$.       

Comparing \cref{f:model-availability-10x} to \cref{f:model-availability}, we can observe how the model availability decreases when nodes spend more time with computing tasks, even if the model sizes are small, so they are not able to exchange their model instances until they have been merged and trained.


The approximation of \cref{eq:approx_2nd} can be of use also in this case for small $L$. It actually reveals that we should expect $\overline{A^{(m)}} = 0.46$, which is very much in line with the result in the figure. However, here the impact of computation and communication bottlenecks, as the number of models increases, is much heavier than in the case of \cref{f:model-availability}.

Model availability values with large $L$ can be also estimated as before: the probability to receive an observation is $0.15$, each observation trains a different model with high probability, and then the node carries the observation during its average residual sojourn time in the \ac{RZ}, which in this case is $T_{\text{RZ}}/2 - (T_M+T_T)$. This implies that the model availability reduces to $0.15 \cdot (282/2 - 25)/282 \simeq 0.062$. This result is in line with what obtained via simulation with any number of models. Zooming into \cref{f:model-availability-10x} at $L=10^8$ b would reveal that the simulation results yield availability $0.062$ for $M=1$, $0.061$ for $M=3$ and $0.055$ for $M=10$, which also indicates that the computing load plays a role, with a slightly detrimental impact on performance, although the effect is minor.


\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{fig/obs-availability-overtime-smallL-10x.pdf}
\caption{Observation availability over time with high training and  merging times and $L=0.01$ Mb.} 
\label{f:smallL-long}
\end{figure}

With long processing times and small $L$, \cref{f:smallL-long} shows that the observation availability evolves more slowly than with short processing time. The figure also clearly shows how the number of models becomes very important. Both phenomena are due to the relevance of computing tasks in this scenario. Here the case with only one model has a load that can be handled by the system, hence its observation availability curve is very similar to the case with low processing times, except for the initial delay due to longer training and merging times. Instead, the curves with 3 and 10 models clearly show that computation has become a bottleneck, and the growth rate of the curves becomes progressively smaller as $M$ grows.
Note that the higher the number of models, the smaller the model availability (see \cref{f:model-availability-10x} for small $L$) and the smaller the number of nodes with model that appears at the denominator of the expression used to compute the observation availability curves. This explains why the curves for $3$ and $10$ models appear to start fast in \cref{f:smallL-long}, although their growing rate is clearly smaller than at $M=1$.

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{fig/obs-availability-overtime-largeL-10x.pdf}
\caption{Observation availability over time with high training and merging times and $L=100$ Mb.} 
\label{f:largeL-long}
\end{figure}

With large $L$, the behavior shown in \cref{f:largeL-long} is qualitatively similar to the one of \cref{f:largeL}, except for the fact that the average number of nodes with model is now smaller, which turns into higher values of instantaneous observation availability. The number of observations alive is however the same in all cases (it is about $\lambda\,\tau_l = 30$ per model), and the differences between the curves with $1$, $3$ and $10$ models in \cref{f:largeL-long} are due to the fact that the average model availability is slightly different in the three cases, as observed in the comment to \cref{f:model-availability-10x}, hence so is the number of nodes in the \ac{RZ} with model, whose inverse value is the observation availability for this case in which only one node carries each observation. In particular, with the model availability at $L=10^8$ b, we should see, on average $9.73$ nodes with model for $M=1$, hence the observation availability should go to $1/9.73 = 0.103$, while with $M=3$ and $M=10$ we should see observation availability values of about $0.104$ and $0.116$. Those values are close to what shown in \cref{f:largeL-long}.    

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{fig/computational-capacity-10x.pdf}
\caption{Learning capacity with high training and merging times. } 
\label{f:computational-capacity-10x}
\end{figure}


Finally, \cref{f:computational-capacity-10x} shows the learning capacity for high computing times $T_T$ and $T_M$. Here, we observe that even if the trend of the curves is similar, the amount of observations at every node, on average, is much lower than in \cref{f:computational-capacity} for all sizes of $L$ but specially for small model sizes. In this case, it is clear that the merging and training times have a significant impact in the computing power of the system and for that reason nodes are not able to retrieve as many observations as in the analyzed case at lower computing load. For low $L$, here the capacity does not scale with the number of models, while it roughly does at high values of $L$. The reason is that with large model sizes the number of observations per model tend to be similar, independently on the number of models, as observed in \cref{f:largeL} and \cref{f:largeL-long}. Note also that the rightmost values of the curves for $\overline{T}$ roughly correspond to the rightmost values of the curves for $\overline{A^{(m)}}$ multiplied by the number of models, as for the case of low processing times. 
Instead, with small model sizes, the computing load---with more than one model and the model availability of \cref{f:model-availability-10x}---becomes high and clogs up the system. For instance, with $10$ models, a node will receive about $1.3$ new instances every $40$~s, which takes at least $80\%$ of its time. This limits the learning capacity of nodes, although not as much as the computing bottleneck does when $L$ grows. Moreover, the impact of computing load is much more gradual than the impact of the \ac{FC} bottleneck, which is still well visible in the figures with high processing time for training and merging.

==> old/4.system_model.tex <==
\section{System Model}
\label{sec:system}


\subsection{Proactive FC computing scheme}

RZ and ZOI are circular and concentric. Nodes which enter the replication zone (RZ) have a set of $T$ different computing tasks, which they have to perform by the time they enter the Zone of Interest (ZOI), a region of the plane within the RZ. All nodes entering the RZ have the same set $T$. We assume nodes enter the RZ with a dataset for each of the computing tasks they have to perform. At each node $i$, for each task $t$ we assume there is a dataset $D_{i,t}$ required to perform the task. $\forall \{t_1,i_1\}, \{t_2,i_2\}$ we assume that $D_{i_1,t_1} \cap D_{i_2,t_2}=  \varnothing$ (this can be relaxed later, but it sounds like conservative).
To each of the $T$ tasks it is associated a \textit{model} $M_t$ i.e. a piece of software and data (e.g. a ML architecture with its parameters) which, together with the user data, are required to execute the $t$-th task on that user.
%Each client node entering the AZ has $T$ computing tasks, to perform by the time it enters the ZOI.
\com{How models are produced and trained is out of the scope of this work. We assume they are in a final state, i.e. they do not need further training (also because here we have no notion of model performance, if one excludes the time it takes to run.)}\\

We assume the computing tasks to be performed are related to a specific spatial context. A typical example is a computing task related to the training or the use of a ML model. In these cases, the model has been built taking into account local data and context, and it is therefore highly specific for that context itself. As we assume no static infrastructure (e.g. edge servers) can support nodes in the computation, these models only reside on nodes (both client and server) and they are made available in a region around the ZOI called the replication zone (RZ) via the FC paradigm. We denote with $L$ the size of a model, i.e. the total amount of info which has to be transferred between two nodes in order to transfer the model.

\vm{This is the first problem tackled in the approach proposed by Gianluca: make the model float, which is not much different from content floating as we have studied and published so far.}\com{Indeed, research problems are not here. This is just a component.} Nodes entering the RZ possess no model. At the beginning of the floating scheme, for each model $t$ we assume there is a subset of the nodes in the RZ which possess it. Every time two nodes meet, each model is replicated from the node who possesses it to the one who doesn't, in a random order. Nodes which exit the RZ discard the models. Nodes have infinite memory size.

As soon as a client node receives the model for the $t-$th task, it starts performing the computing task if no other task is being performed. Otherwise, it waits for the end of the task under execution to start a new one. We assume a node can perform only one computing task at a time. Let $d$ the time required to complete a task.     

The performance metric of this scheme (the \textit{success probability})is the probability for a task to be complete by the time a user enters the ZOI. If a user did not complete the task by the time it enters the ZOI, he will be forced to use cloud services and cellular communications to get it completed. 

\vm{From this point on, this seems another paper, with another research problem. Here the problem is opportunistic offloading, for which there are a lot of results in the literature. What's new here?}
\com{The novelty (small or not) is proactive computing supported by FC-enabled offloading. Offloading is only a component. The old FC scheme, in support of computing, is another (well studied) component. But the whole scheme is new (to the best of my current knowledge).}
We assume that in addition to perform computing tasks locally, using the computing resources of the node itself, nodes can offload the computing task to other client nodes, in order to maximize the success probability. This might happen when  the offloading node has significantly less tasks to complete than the offloaded (e.g. because it has already entered the ZOI), or when the offloading performs computations faster. 
Once the offloading node completes the task, we assume that the result is received instantaneously by the offloaded node, if the two nodes are still in contact. Otherwise, if the two nodes stop being in contact during model/data transfer and offloaded task execution, the offloader discards the computing task.
For this reason (i.e given the limited duration of contacts among nodes), the offloaded tasks take precedence over other tasks of the offloading node.  \vm{I'm confused. Which one is  the offloading node and which the offloader?}
\com{Offloaded node is the node whose load is taken off. The node who helps is the offloading node.}
\vm{Assuming that the offloading node is the one which takes the task and lends compute power to someone else, it is questionable that it would give priority to offloaded tasks over its own tasks. }\com{Very questionable, agree. Already this shows that it is not clear which scheduling strategy works best-an open issue. I assumed that tasks done on behalf of other nodes needs to take precedence, as contacts do not last forever, and if nodes get disconnected while the offloaded task is still not complete I assumed (but we can change this, as well as many other aspects) that the offloaded task get discarded. I am not sure this is actually optimal, in view of the main performance parameter - the mean success probability (or mean probability for a task to be executed before entering the ZOI).}

%If the offloading possesses the model for the task being offloaded, it only needs to receive the dataset from the offloading node relative to that task. Otherwise, the offloading node has to send to the offloader also the model required for that task \com{we can change this, if needed}.
%\com{(When nodes have finite memory for models, we can assume that they are allowed to discard the model for a given task when that task is completed. But let us neglect this in a first step).}
%The second class of nodes is given by the \textit{server nodes}. They do not need to perform computations by their own, but they may perform computation on behalf of client nodes, i.e. play the role of offloaders. Let $k$ be the ratio between the task completion time at client nodes and at server nodes.

At any point in time, every node can communicate with at most another node, and it cannot change the node with which it is communicating until the exchange between the two nodes is complete (i.e. the two nodes have nothing to exchange anymore, and all offloaded tasks have been completed).

The specific task and communications scheduling algorithm is as follows.
Let i and j be the two nodes in contact. 
When node $i$ is done transmitting all the models which are missing by node $j$, node $j$ updates its schedule of tasks to be executed, and computes the time at which all the tasks of the queue will be completed. As we assume to know the mean time to ZOI traversal for each node $j$, conditioned to having spent $\delta$ seconds in the RZ, node $j$ can forecast the average success probability for its own tasks. 
\vm{The forecast introduces a third problem to solve, which is orthogonal to the one of floating the model and the one of offloading the computation.}
\com{Indeed, taken seriously. But we can simplify on this dimension, by assuming (as I have assumed here, see system model) that we know the pdf of the mean time between RZ ingress and ZOI ingress. Then the "forecast" is implemented by estimating the mean time to ZOI ingress, and the time taken to complete all tasks in the queue (which we assume deterministic). }
Node $i$ performs the same forecast. 
Both nodes compute also how such forecasts would change if the node with lower forecasted success rate offloads one or more tasks to the other node, and determine the optimal number of offloaded tasks, 
taking into account the time it takes to transfer the model, and the fact that offloaded tasks take priority over local tasks. \vm{My impression is that this work would deviate a lot form what Noelia has done so far, and there will be no time to complete it before Noelia's contract ends}

\mam{My elaboration on your ideas:
Consider an area where many things happen (e.g., a theme park, like Disneyland or Seaworld, but also a factory floor or a battlefield). Over this area many actors (humans or machines) collect viewpoints of what is happening, but they only have partial information, while global information could be very valuable to make decisions (which attraction to visit, where to provide additional workforce or more soldiers). Global information can only be obtained by collecting and fusing user viewpoints that are progressively updated in the end user terminals. When terminals meet, they exchange their viewpoints and generate a fusion, which becomes more valuable because it incorporates many viewpoints, some older, some more recent. The utility of the newly generated viewpoint is a function of the number of collected individual viewpoints and of their ages. We could investigate the evolution of the average utility of viewpoints (might be called value of information). In the code of Noelia this should not be very difficult to implement. It needs only to keep track of what viewpoints are collected and their ages, so that utility can be computed at any time for all users.}




\com{\textbf{GR My elaborations over MAM.} 
With a system, where info is distributed but where no new info is produced over time, we will see the fusion gradually converging to a global view (complete or not, based on how well the single elements and the fusion float).

If we assume a (stationary) arrival process of new info which has to be fused with new one, the fusion keeps on evolving constantly.

3) if the age of info is in  (i.e, if we have a notion of users regularly producing "updates", we should have a look at  "the age of gossip" paper by JYLB. That would mark a deviation from the traditional FC scheme, as for every content may be floating in its AZ in several different versions, and a node getting two versions would keep and replicate only the most recent one.

The age of gossip paper does not consider 1) conditions for info not to disappear, as a function of system geometry (the anchor zone) and node mobility; 2)  a notion of maximum load of information which the system can support (similar to FC capacity idea ), and the relationship (trade-off) between such a maximum load and the mean age of floating information. This is to me another potential direction of work, which would elaborate on top of JYLB paper.}




==> vanilla_algorithm.tex <==
\subsection{Scheduling, version 1}
% Every node has to contribute to a performance goal (complete all computing tasks by the time it enters the ZOI) and to the model floating scheme.
% As a node is free from computing tasks duties once it has entered the ZOI, we assume that when two nodes meet, task completion takes priority over model exchanges for the sake of model floating.

As for task completion, a specific algorithm must be defined. Take two nodes, $a$ and $b$, which come in contact. For each task $t$, let $p_t$ be the probability that they possess the model for that task, and $c_t$ the probability that the task has been completed by the time the two nodes come in contact. Hence every node has a list of tasks which are not complete yet, either because they had no time to do so, or because they have no model for that task.

For each task for which they possess the model, they have to decide whether to execute it locally, or propose to offload it to the other node (if the other node has the model for that task, of course). They might decide to do so to parallelize and hence get more tasks completed for them in a same time interval, but this might come at the expense of the other node's ability to complete its own tasks.

In a first try, we assume nodes offload only when the offloader has no tasks of its own to complete.

Hence we distinguish two cases:
\begin{itemize}
    \item Both nodes have own tasks to complete. In this case, nodes transfer models (if they have them) in order to enable the other node to complete its own tasks. Order is random among all models which need to be exchanged. When done, node transfer missing models at the other node (note well: a node might have tasks completed because of offloading, hence without ever having possessed a model for them).
    \item Only one of the two nodes has tasks to complete. Then the offloading node (the one with open tasks) starts sending to the offloader all tasks ( i e. the datasets) for which the offloading has no model (we call this type a tasks). In parallel, it puts on a list those open tasks for which it has a model (type b tasks), and it starts executing them in sequence, starting from the top of the list. If the offloader is done with type a tasks, it starts executing type a tasks, starting from the bottom of the list up, until either all tasks are completed, or contact time is over. When either of the two nodes is done with the task execution process, it starts transferring missing models at the other node.
\end{itemize}

\com{This is only one of the many possible scheduling strategies. I hope I can make it into differential equations.}


\subsection{Scheduling, version 2}
Notation:
\begin{itemize}
    \item $t_i$ the time at which the $i-th$ node enters the RZ; 
    \item $\tau_i(t)$ the residual time until the $i-th$ node enters the ZOI. It is a random variable of which we assume to know its PDF, induced by mobility patterns and geometry of the RZ and ZOI. Let $\bar{\tau}_i(t)$ be its mean; 
    \item $\t^c_i(t)$ the amount of time required by the $i-th$ node to complete all the computing tasks which are scheduled at that node at time $t$. This includes both own tasks and tasks taken from other nodes.
    \item $d_o$ is the expected time interval from an offloading decision until the offloaded task is completed. It is the sum of the time taken to complete the task, plus the max between the time taken to transmit task and data to the other node, and the time taken by the eventual running task to complete.  
\end{itemize}

Consider two nodes labelled as $i$ and $j$, coming in contact at time $t_o$ in the RZ. Scheduling happens separately for each direction of transmission.
Let us consider first node $i$.
\begin{itemize}
    \item Firstly, it sends to node $j$ all models which it does not possess.
    \item At the same time, node $i$ starts (or continues) to execute the tasks in its own queue. The local tasks are scheduled in random order. If at any time it receives one or more offloaded tasks, it places them in its queue at a higher priority than local tasks.
    \item Let $t$ be the time at which the last model is sent at node $j$. 
\end{itemize}







Assume that $\t^c_i(t)>\t^c_j(t)+d_o$.
Then node $i$ can offload to node $j$. Let  $\t'^c_i(t)$ and $\t'^c_i(t)$ the new amount of time required at the two nodes to complete all computing tasks. Then the amount of offloaded tasks is the maximum amount for which $\t'^c_i(t)>\t'^c_j(t)$. 





If a node takes over a task from another one, that task has higher priority over its own tasks, as successful completion of offloaded tasks is also a function of contact duration, which is limited. However this priority is non preemptive (i.e. it does not prevent completion of a running task).  










As a node is free from computing tasks duties once it has entered the ZOI, we assume that when two nodes meet, task completion takes priority over model exchanges for the sake of model floating.

As for task completion, a specific algorithm must be defined. Take two nodes, $a$ and $b$, which come in contact. For each task $t$, let $p_t$ be the probability that they possess the model for that task, and $c_t$ the probability that the task has been completed by the time the two nodes come in contact. Hence every node has a list of tasks which are not complete yet, either because they had no time to do so, or because they have no model for that task.

For each task for which they possess the model, they have to decide whether to execute it locally, or propose to offload it to the other node (if the other node has the model for that task, of course). They might decide to do so to parallelize and hence get more tasks completed for them in a same time interval, but this might come at the expense of the other node's ability to complete its own tasks.

In a first try, we assume nodes offload only when the offloader has no tasks of its own to complete.

Hence we distinguish two cases:
\begin{itemize}
    \item Both nodes have own tasks to complete. In this case, nodes transfer models (if they have them) in order to enable the other node to complete its own tasks. Order is random among all models which need to be exchanged. When done, node transfer missing models at the other node (note well: a node might have tasks completed because of offloading, hence without ever having possessed a model for them).
    \item Only one of the two nodes has tasks to complete. Then the offloading node (the one with open tasks) starts sending to the offloader all tasks ( i e. the datasets) for which the offloading has no model (we call this type a tasks). In parallel, it puts on a list those open tasks for which it has a model (type b tasks), and it starts executing them in sequence, starting from the top of the list. If the offloader is done with type a tasks, it starts executing type a tasks, starting from the bottom of the list up, until either all tasks are completed, or contact time is over. When either of the two nodes is done with the task execution process, it starts transferring missing models at the other node.
\end{itemize}

\com{This is only one of the many possible scheduling strategies. I hope I can make it into differential equations.}



\subsection{Performance issues}

Conditions for models to float are the same as usual. 

The performance parameter here is, for every task, the ratio of nodes which enter the ZOI while having completed the task (success rate), or equivalently, the mean number of completed tasks at the moment of entering the ZOI.

Some function of the mean number of completed task per entering node, and of the rate at which nodes enter the ZOI (maybe simply the product of the two?) is a measure of the overall "computing power" of the system, i.e. of how much it is able to offload cloud or static edge servers (which we can imagine are to be employed when the system fails, i.e. for every task not completed by the time the node enters the ZOI). 

The relevant performance aspect here are related to the characterization of the tradeoff between host memory, computing and communications. With an appropriate energy model for each node, energy budget could also come into the mix.

In addition to the classical approach for model floating (nothing new there, except for the fact that a model might be replicated in the context of an offloading operation, too), the differential equations here have to express the mean success rate of a task (i.e. the mean fraction of nodes in the RZ which have completed the task). This can be done with a nonspatial model (the usual MF limit) only, or complemented by a spatial one, possibly based on the knowledge of 1) the likelihood for a node to transit through the ZOI, and 2) the PDF of the time between RZ ingress and entrance to the ZOI.
Formulating 2) in this way could allow us to avoid doing works such as those done with Shahzad, in which these spatial features were tied to a specific mobility (e.g. RD).



